Infinity category theory from scratch

We use the terms "$\infty$-categories" and "$\infty$-functors" to mean the objects and morphisms in an "$\infty$-cosmos." Quasi-categories, Segal categories, complete Segal spaces, naturally marked simplicial sets, iterated complete Segal spaces, $\theta_n$-spaces, and fibered versions of each of these are all $\infty$-categories in this sense. We show that the basic category theory of $\infty$-categories and $\infty$-functors can be developed from the axioms of an $\infty$-cosmos; indeed, most of the work is internal to a strict 2-category of $\infty$-categories, $\infty$-functors, and natural transformations. In the $\infty$-cosmos of quasi-categories, we recapture precisely the same theory developed by Joyal and Lurie, although in most cases our definitions, which are 2-categorical rather than combinatorial in nature, present a new incarnation of the standard concepts. In the first lecture, we define an $\infty$-cosmos and introduce its "homotopy 2-category," using formal category theory to define and study equivalences and adjunctions between $\infty$-categories. In the second lecture, we study (co)limits of diagrams taking values in an $\infty$-category and the relationship between (co)limits and adjunctions. In the third lecture, we introduce comma $\infty$-categories, which are used to encode the universal properties of (co)limits and adjointness and prove "model independence" results. In the fourth lecture, we introduce (co)cartesian fibrations, describe the calculus of "modules" between $\infty$-categories, and use this framework to prove the Yoneda lemma and develop the theory of pointwise Kan extensions of $\infty$-functors.

==> cohadj_lab.tex <==
\newlabel{cohadj:sec:intro-adj-data}{{1.1}{2}{Adjunction data}{subsection.1.1}{}}
\newlabel{cohadj:eq:sampletriangleidentities}{{1.1.1}{3}{Adjunction data}{equation.1.1.1}{}}
\newlabel{cohadj:eq:horn-1}{{1.1.2}{3}{Adjunction data}{equation.1.1.2}{}}
\newlabel{cohadj:eq:middle.four}{{1.1.3}{4}{Adjunction data}{equation.1.1.3}{}}
\newlabel{cohadj:eq:horn-2}{{1.1.4}{4}{Adjunction data}{equation.1.1.4}{}}
\newlabel{cohadj:sec:computads}{{2}{7}{Simplicial computads}{section.2}{}}
\newlabel{cohadj:subsec:computads}{{2.1}{7}{Simplicial categories and simplicial computads}{subsection.2.1}{}}
\newlabel{cohadj:ntn:whiskering}{{2.1.2}{8}{whiskering in a simplicial category}{thm.2.1.2}{}}
\newlabel{cohadj:ntn:generic-cattwo}{{2.1.3}{8}{the generic $n$-arrow}{thm.2.1.3}{}}
\newlabel{cohadj:defn:computads}{{2.1.4}{8}{(relative) simplicial computads}{thm.2.1.4}{}}
\newlabel{cohadj:obs:simp-computad-char}{{2.1.5}{8}{an explicit characterisation of simplicial computads}{thm.2.1.5}{}}
\newlabel{cohadj:eq:computad-arrrow-decomp}{{2.1.6}{9}{an explicit characterisation of simplicial computads}{equation.2.1.6}{}}
\newlabel{cohadj:ex:gothic-C}{{2.1.10}{9}{}{thm.2.1.10}{}}
\newlabel{cohadj:ex:homotopy-coherent-simplex}{{2.1.11}{10}{}{thm.2.1.11}{}}
\newlabel{cohadj:subsec:subcomputads}{{2.2}{10}{Simplicial subcomputads}{subsection.2.2}{}}
\newlabel{cohadj:ex:mono-subcomputad}{{2.2.3}{10}{}{thm.2.2.3}{}}
\newlabel{cohadj:defn:generated-subcomputad}{{2.2.4}{11}{}{thm.2.2.4}{}}
\newlabel{cohadj:ex:simp-cat.(co)skeleta}{{2.2.5}{11}{(co)skeleta of simplicial categories}{thm.2.2.5}{}}
\newlabel{cohadj:prop:simp-computad-maps}{{2.2.6}{11}{}{thm.2.2.6}{}}
\newlabel{cohadj:sec:generic-adj}{{3}{12}{The generic adjunction}{section.3}{}}
\newlabel{cohadj:ssec:graphical}{{3.1}{12}{A graphical calculus for the simplicial category \protect \texorpdfstring {$\protect \Adj $}{Adj}}{subsection.3.1}{}}
\newlabel{cohadj:eq:samplesquiggle}{{3.1.1}{13}{A graphical calculus for the simplicial category \protect \texorpdfstring {$\protect \Adj $}{Adj}}{equation.3.1.1}{}}
\newlabel{cohadj:def:strict-und-squiggles}{{3.1.2}{14}{strictly undulating squiggles}{thm.3.1.2}{}}
\newlabel{cohadj:item:strict-und-squiggle-1}{{{{(i)}}}{14}{strictly undulating squiggles}{Item.1}{}}
\newlabel{cohadj:item:strict-und-squiggle-2}{{{{(ii)}}}{14}{strictly undulating squiggles}{Item.2}{}}
\newlabel{cohadj:item:und-squiggle-2}{{{{(ii)$'$}}}{14}{strictly undulating squiggles}{Item.3}{}}
\newlabel{cohadj:def:comp-squiggles}{{3.1.3}{14}{composing squiggles}{thm.3.1.3}{}}
\newlabel{cohadj:eq:samplesquiggle2}{{3.1.6}{15}{simplicial action on strictly undulating squiggles}{equation.3.1.6}{}}
\newlabel{cohadj:obs:interval.rep}{{3.1.7}{17}{interval representation}{thm.3.1.7}{}}
\newlabel{cohadj:obs:squiggle-vertices}{{3.1.9}{18}{the vertices of an arrow in $\Adj $}{thm.3.1.9}{}}
\newlabel{cohadj:prop:adjcomputad}{{3.1.10}{19}{}{thm.3.1.10}{}}
\newlabel{cohadj:ex:sample-adjunction-data}{{3.1.11}{19}{adjunction data in $\Adj $}{thm.3.1.11}{}}
\newlabel{cohadj:eq:ualpha-faces}{{3.1.12}{20}{adjunction data in $\Adj $}{equation.3.1.12}{}}
\newlabel{cohadj:ssec:2-cat-adj}{{3.2}{21}{The simplicial category \texorpdfstring {$\protect \Adj $}{Adj} as a 2-category}{subsection.3.2}{}}
\newlabel{cohadj:prop:adj.2-cat}{{3.2.2}{21}{}{thm.3.2.2}{}}
\newlabel{cohadj:eq:samplesquiggles4}{{3.2.3}{21}{The simplicial category \texorpdfstring {$\protect \Adj $}{Adj} as a 2-category}{equation.3.2.3}{}}
\newlabel{cohadj:eq:samplesquiggle3}{{3.2.4}{22}{The simplicial category \texorpdfstring {$\protect \Adj $}{Adj} as a 2-category}{equation.3.2.4}{}}
\newlabel{cohadj:rmk:hammock}{{3.2.5}{22}{}{thm.3.2.5}{}}
\newlabel{cohadj:eq:karol}{{3.2.6}{23}{}{equation.3.2.6}{}}
\newlabel{cohadj:ssec:adj-is-adj}{{3.3}{23}{The 2-categorical universal property of \protect \texorpdfstring {$\protect \Adj $}{Adj}}{subsection.3.3}{}}
\newlabel{cohadj:obs:2-cat.as.simp-cat}{{3.3.1}{24}{2-categories as simplicial categories}{thm.3.3.1}{}}
\newlabel{cohadj:eq:genadjdata}{{3.3.3}{24}{the adjunction in \protect \texorpdfstring {$\protect \Adj $}{Adj}}{equation.3.3.3}{}}
\newlabel{cohadj:prop:2-cat-univ-Adj}{{3.3.4}{24}{a 2-categorical universal property of \protect \texorpdfstring {$\protect \Adj $}{Adj}}{thm.3.3.4}{}}
\newlabel{cohadj:cor:schanuel-street-iso}{{3.3.5}{25}{}{thm.3.3.5}{}}
\newlabel{cohadj:obs:delta.adj.duality}{{3.3.6}{26}{adjunctions in \protect \texorpdfstring {$\protect \Del +$}{Delta+}}{thm.3.3.6}{}}
\newlabel{cohadj:eq:elem.op.adj}{{3.3.7}{26}{adjunctions in \protect \texorpdfstring {$\protect \Del +$}{Delta+}}{equation.3.3.7}{}}
\newlabel{cohadj:rmk:schanuel-street}{{3.3.8}{26}{the Schanuel and Street 2-category $\Adj $}{thm.3.3.8}{}}
\newlabel{cohadj:sec:adjunction-data}{{4}{28}{Adjunction data}{section.4}{}}
\newlabel{cohadj:ssec:fillable}{{4.1}{28}{Fillable arrows}{subsection.4.1}{}}
\newlabel{cohadj:obs:fillable-dist-face}{{4.1.2}{29}{fillable arrows and distinguished faces}{thm.4.1.2}{}}
\newlabel{cohadj:lem:fillablecodim1}{{4.1.3}{29}{}{thm.4.1.3}{}}
\newlabel{cohadj:lem:fillablecodim1'}{{4.1.4}{30}{}{thm.4.1.4}{}}
\newlabel{cohadj:ssec:parental}{{4.2}{30}{Parental subcomputads}{subsection.4.2}{}}
\newlabel{cohadj:defn:parental-subcomputad}{{4.2.2}{30}{parental subcomputads of $\Adj $}{thm.4.2.2}{}}
\newlabel{cohadj:ex:parental-subcomputad}{{4.2.3}{31}{}{thm.4.2.3}{}}
\newlabel{cohadj:ex:non-parental-subcomputad}{{4.2.4}{31}{a non-example}{thm.4.2.4}{}}
\newlabel{cohadj:ex:another-parental-subcomputad}{{4.2.5}{31}{}{thm.4.2.5}{}}
\newlabel{cohadj:ntn:generic-catthree}{{4.2.6}{31}{}{thm.4.2.6}{}}
\newlabel{cohadj:eq:3[i]-square}{{4.2.7}{32}{}{equation.4.2.7}{}}
\newlabel{cohadj:def:funct-for-fillable}{{4.2.9}{32}{}{thm.4.2.9}{}}
\newlabel{cohadj:lem:ext-par-subcomp}{{4.2.10}{32}{extending parental subcomputads}{thm.4.2.10}{}}
\newlabel{cohadj:eq:parental-adj-pushout-1}{{4.2.11}{33}{extending parental subcomputads}{equation.4.2.11}{}}
\newlabel{cohadj:eq:parental-adj-pushout-2}{{4.2.12}{33}{extending parental subcomputads}{equation.4.2.12}{}}
\newlabel{cohadj:cor:ext-par-subcomp}{{4.2.13}{34}{}{thm.4.2.13}{}}
\newlabel{cohadj:eq:big-pushout}{{4.2.14}{34}{}{equation.4.2.14}{}}
\newlabel{cohadj:prop:ext-par-subcomp}{{4.2.15}{34}{}{thm.4.2.15}{}}
\newlabel{cohadj:itm:one}{{{{(i)}}}{34}{}{Item.4}{}}
\newlabel{cohadj:itm:two}{{{{(ii)}}}{34}{}{Item.5}{}}
\newlabel{cohadj:ssec:hocoh}{{4.3}{36}{Homotopy Coherent Adjunctions}{subsection.4.3}{}}
\newlabel{cohadj:obs:adjunctions-in-qcat-cats}{{4.3.2}{36}{adjunctions in a quasi-categorically enriched category}{thm.4.3.2}{}}
\newlabel{cohadj:obs:int-univ}{{4.3.4}{37}{the internal universal property of the counit}{thm.4.3.4}{}}
\newlabel{cohadj:lem:rel-lift-terminal}{{4.3.5}{38}{a relative universal property of terminal objects}{thm.4.3.5}{}}
\newlabel{cohadj:prop:rel-int-univ}{{4.3.6}{39}{the relative internal universal property of the counit}{thm.4.3.6}{}}
\newlabel{cohadj:obs:ext-quasicat-homs}{{4.3.7}{39}{}{thm.4.3.7}{}}
\newlabel{cohadj:thm:hty-coherence-exist}{{4.3.8}{40}{}{thm.4.3.8}{}}
\newlabel{cohadj:thm:hty-coherence-exist-I}{{4.3.9}{41}{homotopy coherence of adjunctions I}{thm.4.3.9}{}}
\newlabel{cohadj:thm:hty-coherence-exist-II}{{4.3.11}{42}{homotopy coherence of adjunctions II}{thm.4.3.11}{}}
\newlabel{cohadj:def:adjunction-data}{{4.3.13}{42}{}{thm.4.3.13}{}}
\newlabel{cohadj:ssec:uniqueness}{{4.4}{42}{Homotopical uniqueness of homotopy coherent adjunctions}{subsection.4.4}{}}
\newlabel{cohadj:obs:icon-defn}{{4.4.1}{43}{simplicial enrichment of simplicial categories}{thm.4.4.1}{}}
\newlabel{cohadj:lem:isofib-icon}{{4.4.2}{43}{}{thm.4.4.2}{}}
\newlabel{cohadj:lem:conservative-icon}{{4.4.4}{45}{}{thm.4.4.4}{}}
\newlabel{cohadj:lem:cohadj.space.Kan}{{4.4.6}{46}{}{thm.4.4.6}{}}
\newlabel{cohadj:prop:hty-uniqueness}{{4.4.7}{46}{}{thm.4.4.7}{}}
\newlabel{cohadj:eq:trans-lift-prob-1}{{4.4.8}{47}{Homotopical uniqueness of homotopy coherent adjunctions}{equation.4.4.8}{}}
\newlabel{cohadj:obs:epsilon-icon-expl}{{4.4.9}{47}{}{thm.4.4.9}{}}
\newlabel{cohadj:thm:hty-uniqueness-I}{{4.4.11}{48}{}{thm.4.4.11}{}}
\newlabel{cohadj:prop:counits-proj-trivial}{{4.4.12}{48}{}{thm.4.4.12}{}}
\newlabel{cohadj:lem:fib-contract-fibres}{{4.4.13}{48}{}{thm.4.4.13}{}}
\newlabel{cohadj:prop:leftadjs-proj-trivial}{{4.4.17}{49}{}{thm.4.4.17}{}}
\newlabel{cohadj:thm:hty-uniqueness-II}{{4.4.18}{50}{}{thm.4.4.18}{}}
\newlabel{cohadj:sec:weighted}{{5}{50}{Weighted limits in \protect \texorpdfstring {$\protect \qCat _\infty $}{qCat}}{section.5}{}}
\newlabel{cohadj:subsec:weighted}{{5.1}{50}{Weighted limits and colimits}{subsection.5.1}{}}
\newlabel{cohadj:defn:cotensors}{{5.1.1}{50}{cotensors}{thm.5.1.1}{}}
\newlabel{cohadj:eq:wlimformula}{{5.1.3}{51}{weighted limits}{equation.5.1.3}{}}
\newlabel{cohadj:eq:wlim-def-prop}{{5.1.4}{51}{weighted limits}{equation.5.1.4}{}}
\newlabel{cohadj:ex:rep-weights}{{5.1.5}{51}{representable weights}{thm.5.1.5}{}}
\newlabel{cohadj:eq:yoneda}{{5.1.6}{51}{representable weights}{equation.5.1.6}{}}
\newlabel{cohadj:obs:weighted-cocontinuity}{{5.1.7}{51}{}{thm.5.1.7}{}}
\newlabel{cohadj:ex:diagrams-weighted-limit}{{5.1.8}{52}{diagrams}{thm.5.1.8}{}}
\newlabel{cohadj:ex:commaweightedlimit}{{5.1.9}{52}{comma quasi-categories}{thm.5.1.9}{}}
\newlabel{cohadj:ex:homotopyweighted}{{5.1.10}{52}{homotopy limits as weighted limits}{thm.5.1.10}{}}
\newlabel{cohadj:lem:lanweights}{{5.1.11}{52}{weighted limits and Kan extensions}{thm.5.1.11}{}}
\newlabel{cohadj:subsec:weighted-qcat}{{5.2}{53}{Weighted limits in the quasi-categorical context}{subsection.5.2}{}}
\newlabel{cohadj:defn:proj-cof}{{5.2.1}{53}{projective cofibrations}{thm.5.2.1}{}}
\newlabel{cohadj:prop:projwlims2}{{5.2.2}{53}{}{thm.5.2.2}{}}
\newlabel{cohadj:eq:layer-in-tower}{{5.2.3}{53}{Weighted limits in the quasi-categorical context}{equation.5.2.3}{}}
\newlabel{cohadj:prop:projwlims}{{5.2.4}{54}{}{thm.5.2.4}{}}
\newlabel{cohadj:prop:proj-wlim-homotopical}{{5.2.6}{54}{}{thm.5.2.6}{}}
\newlabel{cohadj:rmk:projwlims}{{5.2.7}{54}{}{thm.5.2.7}{}}
\newlabel{cohadj:rmk:categories-special-case}{{5.2.9}{55}{2-categorical weighted limits and quasi-categorical weighted limits}{thm.5.2.9}{}}
\newlabel{cohadj:subsec:collage}{{5.3}{55}{The collage construction}{subsection.5.3}{}}
\newlabel{cohadj:obs:coll-right-adj}{{5.3.2}{55}{a right adjoint to the collage construction}{thm.5.3.2}{}}
\newlabel{cohadj:prop:projcofchar2}{{5.3.3}{56}{}{thm.5.3.3}{}}
\newlabel{cohadj:eq:pushout-transform}{{5.3.4}{56}{The collage construction}{equation.5.3.4}{}}
\newlabel{cohadj:prop:projcofchar}{{5.3.5}{58}{}{thm.5.3.5}{}}
\newlabel{cohadj:sec:formal}{{6}{58}{The formal theory of homotopy coherent monads}{section.6}{}}
\newlabel{cohadj:ssec:formalmonads}{{6.1}{59}{Weighted limits for the formal theory of monads}{subsection.6.1}{}}
\newlabel{cohadj:obs:mnd-weights}{{6.1.3}{59}{weights on $\Mnd $}{thm.6.1.3}{}}
\newlabel{cohadj:defn:W+}{{6.1.4}{60}{monad resolutions}{thm.6.1.4}{}}
\newlabel{cohadj:eq:resolution2}{{6.1.5}{60}{monad resolutions}{equation.6.1.5}{}}
\newlabel{cohadj:defn:W-}{{6.1.6}{61}{}{thm.6.1.6}{}}
\newlabel{cohadj:defn:EMobject}{{6.1.7}{61}{quasi-category of algebras}{thm.6.1.7}{}}
\newlabel{cohadj:lem:projcof1}{{6.1.8}{61}{}{thm.6.1.8}{}}
\newlabel{cohadj:rmk:expl-htycoh-alg}{{6.1.10}{61}{}{thm.6.1.10}{}}
\newlabel{cohadj:eq:expl-htycoh-alg-cond}{{6.1.11}{61}{}{equation.6.1.11}{}}
\newlabel{cohadj:eq:algebraresolution}{{6.1.12}{62}{}{equation.6.1.12}{}}
\newlabel{cohadj:ex:monadicadj}{{6.1.14}{63}{monadic adjunction}{thm.6.1.14}{}}
\newlabel{cohadj:eq:monadicadjunctionweights}{{6.1.15}{63}{monadic adjunction}{equation.6.1.15}{}}
\newlabel{cohadj:ssec:monadicequivs}{{6.2}{63}{Conservativity of the monadic forgetful functor}{subsection.6.2}{}}
\newlabel{cohadj:prop:conservative-char}{{6.2.2}{63}{}{thm.6.2.2}{}}
\newlabel{cohadj:cor:uTconservative}{{6.2.3}{64}{}{thm.6.2.3}{}}
\newlabel{cohadj:obs:understanding-monadic-forgetful-functor}{{6.2.4}{64}{}{thm.6.2.4}{}}
\newlabel{cohadj:rmk:u-map}{{6.2.5}{65}{}{thm.6.2.5}{}}
\newlabel{cohadj:ssec:algcolims}{{6.3}{65}{Colimit representation of algebras}{subsection.6.3}{}}
\newlabel{cohadj:eq:splitcoeq}{{6.3.1}{65}{Colimit representation of algebras}{equation.6.3.1}{}}
\newlabel{cohadj:eq:splitgeorealizations}{{6.3.2}{66}{}{equation.6.3.2}{}}
\newlabel{cohadj:rec:splitgeorealizations}{{6.3.3}{66}{constructing the triangle in theorem \refI {thm:splitgeorealizations}}{thm.6.3.3}{}}
\newlabel{cohadj:eq:canonical-2-cell}{{6.3.4}{66}{constructing the triangle in theorem \refI {thm:splitgeorealizations}}{equation.6.3.4}{}}
\newlabel{cohadj:defn:u-split-aug}{{6.3.5}{66}{$u$-split augmented simplicial objects}{thm.6.3.5}{}}
\newlabel{cohadj:eq:u-split-pullback}{{6.3.6}{67}{$u$-split augmented simplicial objects}{equation.6.3.6}{}}
\newlabel{cohadj:prop:uTcreates}{{6.3.7}{67}{}{thm.6.3.7}{}}
\newlabel{cohadj:thm:uTcreates}{{6.3.8}{67}{}{thm.6.3.8}{}}
\newlabel{cohadj:obs:uTcreates}{{6.3.9}{67}{}{thm.6.3.9}{}}
\newlabel{cohadj:eq:colim.diag.1}{{6.3.10}{67}{}{equation.6.3.10}{}}
\newlabel{cohadj:eq:colimit-diag-ut-split}{{6.3.11}{69}{Colimit representation of algebras}{equation.6.3.11}{}}
\newlabel{cohadj:eq:colimit-diag-ut-split-under}{{6.3.12}{69}{Colimit representation of algebras}{equation.6.3.12}{}}
\newlabel{cohadj:eq:Wscdefn}{{6.3.14}{70}{a direct description of $S(u^t)$}{equation.6.3.14}{}}
\newlabel{cohadj:obs:canonical.alg.pres}{{6.3.15}{70}{}{thm.6.3.15}{}}
\newlabel{cohadj:eq:usplitpushout}{{6.3.16}{70}{}{equation.6.3.16}{}}
\newlabel{cohadj:thm:colim-rep-algebras}{{6.3.17}{71}{canonical colimit representation of algebras}{thm.6.3.17}{}}
\newlabel{cohadj:eq:canonical-colimits}{{6.3.18}{71}{canonical colimit representation of algebras}{equation.6.3.18}{}}
\newlabel{cohadj:eq:downstairs-colimit}{{6.3.19}{71}{canonical colimit representation of algebras}{equation.6.3.19}{}}
\newlabel{cohadj:sec:monadicity}{{7}{72}{Monadicity}{section.7}{}}
\newlabel{cohadj:ssec:comparison}{{7.1}{72}{Comparison with the monadic adjunction}{subsection.7.1}{}}
\newlabel{cohadj:lem:actionquotient}{{7.1.3}{73}{}{thm.7.1.3}{}}
\newlabel{cohadj:eq:actionquotient}{{7.1.4}{73}{}{equation.7.1.4}{}}
\newlabel{cohadj:obs:lanW-}{{7.1.5}{73}{}{thm.7.1.5}{}}
\newlabel{cohadj:eq:monadicadjunctionweight}{{7.1.6}{74}{}{equation.7.1.6}{}}
\newlabel{cohadj:eq:monadiccomparison}{{7.1.10}{74}{comparison with the monadic adjunction}{equation.7.1.10}{}}
\newlabel{cohadj:ssec:monadicity}{{7.2}{74}{The monadicity theorem}{subsection.7.2}{}}
\newlabel{cohadj:eq:usplit}{{7.2.2}{75}{$u$-split simplicial objects}{equation.7.2.2}{}}
\newlabel{cohadj:eq:usplithyp}{{7.2.3}{75}{$u$-split simplicial objects}{equation.7.2.3}{}}
\newlabel{cohadj:thm:monadiccomparisonadj}{{7.2.4}{75}{monadicity I}{thm.7.2.4}{}}
\newlabel{cohadj:eq:Ldefn}{{7.2.5}{75}{The monadicity theorem}{equation.7.2.5}{}}
\newlabel{cohadj:eq:Labs-lifting}{{7.2.6}{76}{The monadicity theorem}{equation.7.2.6}{}}
\newlabel{cohadj:thm:monadicity}{{7.2.7}{77}{monadicity II}{thm.7.2.7}{}}
\newlabel{cohadj:tocindent-1}{0pt}
\newlabel{cohadj:tocindent0}{15.01021pt}
\newlabel{cohadj:tocindent1}{20.88377pt}
\newlabel{cohadj:tocindent2}{34.49158pt}
\newlabel{cohadj:tocindent3}{0pt}


==> complete_lab.tex <==
\newlabel{complete:thm:limits-in-limits}{{1.1}{2}{}{thm.1.1}{}}
\newlabel{complete:item:stepI}{{{{(I)}}}{4}{Outline of the proof}{Item.1}{}}
\newlabel{complete:item:stepII}{{{{(II)}}}{4}{Outline of the proof}{Item.2}{}}
\newlabel{complete:sec:weighted}{{2}{5}{Weighted limits in \texorpdfstring {$\protect \qCat _\infty $}{qCat}}{section.2}{}}
\newlabel{complete:sec:terminal}{{3}{6}{Quasi-categories with terminal objects}{section.3}{}}
\newlabel{complete:defn:qCat-X}{{3.1}{6}{}{thm.3.1}{}}
\newlabel{complete:obs:terminal-pres-banal}{{3.2}{6}{}{thm.3.2}{}}
\newlabel{complete:obs:terminals-in-limits-prf}{{3.3}{6}{}{thm.3.3}{}}
\newlabel{complete:rmk:qCat-term-closure-expl}{{3.4}{7}{proof-schema}{thm.3.4}{}}
\newlabel{complete:enum:term-in-lim-p1}{{{{(i)}}}{7}{proof-schema}{Item.13}{}}
\newlabel{complete:enum:term-in-lim-p2}{{{{(ii)}}}{7}{proof-schema}{Item.14}{}}
\newlabel{complete:rec:terminal.char}{{3.5}{7}{terminal objects}{thm.3.5}{}}
\newlabel{complete:lem:rel-lift-terminal-conv}{{3.7}{8}{}{thm.3.7}{}}
\newlabel{complete:lem:rel-lift-terminal-companion}{{3.8}{8}{}{thm.3.8}{}}
\newlabel{complete:lem:qCat_t-closed-products}{{3.9}{8}{}{thm.3.9}{}}
\newlabel{complete:eq:to-solve-prod}{{3.10}{9}{Conical limits in \texorpdfstring {$\protect \qCat _\emptyset $}{qCat}}{equation.3.10}{}}
\newlabel{complete:lem:qCat_t-closed-pullbacks}{{3.11}{9}{}{thm.3.11}{}}
\newlabel{complete:eq:pb-in-qCat}{{3}{9}{Conical limits in \texorpdfstring {$\protect \qCat _\emptyset $}{qCat}}{thm.3.11}{}}
\newlabel{complete:eq:to-solve-pb}{{3.12}{9}{Conical limits in \texorpdfstring {$\protect \qCat _\emptyset $}{qCat}}{equation.3.12}{}}
\newlabel{complete:lem:qCat_t-closed-countable-composite}{{3.13}{10}{}{thm.3.13}{}}
\newlabel{complete:eq:to-solve-tower}{{3.14}{10}{Conical limits in \texorpdfstring {$\protect \qCat _\emptyset $}{qCat}}{equation.3.14}{}}
\newlabel{complete:lem:qCat_t-closed-idempotents}{{3.15}{11}{}{thm.3.15}{}}
\newlabel{complete:thm:terminal-closure}{{3.16}{11}{}{thm.3.16}{}}
\newlabel{complete:sec:absolute}{{4}{12}{Absolute lifting diagrams via terminal objects}{section.4}{}}
\newlabel{complete:eq:obj-qCat-pbshape}{{4.2}{12}{}{equation.4.2}{}}
\newlabel{complete:eq:obj-qCat-pbshape-trans}{{4.3}{12}{}{equation.4.3}{}}
\newlabel{complete:eq:lifting.triangle}{{4.4}{12}{}{equation.4.4}{}}
\newlabel{complete:defn:abs-lift-trans-right-exactness}{{4.5}{13}{}{thm.4.5}{}}
\newlabel{complete:eq:induced-mate}{{4.6}{13}{}{equation.4.6}{}}
\newlabel{complete:obs:comparison-2cell-composite}{{4.8}{13}{}{thm.4.8}{}}
\newlabel{complete:prop:abslifts-in-limits}{{4.9}{14}{}{thm.4.9}{}}
\newlabel{complete:eq:limit-X-pbshape}{{4.10}{14}{Projective cofibrant weighted limits in \texorpdfstring {$\protect \qCat _{r\infty }^{\protect \pbshape }$}{qCat}}{equation.4.10}{}}
\newlabel{complete:eq:limit-X-pbshape-trans}{{4.11}{14}{Projective cofibrant weighted limits in \texorpdfstring {$\protect \qCat _{r\infty }^{\protect \pbshape }$}{qCat}}{equation.4.11}{}}
\newlabel{complete:obs:comma-simp-functor}{{4.12}{15}{}{thm.4.12}{}}
\newlabel{complete:obs:pointwise-exactness}{{4.13}{15}{a pointwise characterisation of right exactness}{thm.4.13}{}}
\newlabel{complete:lem:right-exact-pointwise}{{4.14}{16}{}{thm.4.14}{}}
\newlabel{complete:lem:conical-closure}{{4.15}{16}{}{thm.4.15}{}}
\newlabel{complete:eq:conical-limit-cone}{{4.16}{17}{Projective cofibrant weighted limits in \texorpdfstring {$\protect \qCat _{r\infty }^{\protect \pbshape }$}{qCat}}{equation.4.16}{}}
\newlabel{complete:lem:cotensor-closure}{{4.17}{18}{}{thm.4.17}{}}
\newlabel{complete:eq:cotensor-in-qCat-pb}{{4.18}{18}{Projective cofibrant weighted limits in \texorpdfstring {$\protect \qCat _{r\infty }^{\protect \pbshape }$}{qCat}}{equation.4.18}{}}
\newlabel{complete:eq:induced-into-cotensor}{{4.19}{19}{Projective cofibrant weighted limits in \texorpdfstring {$\protect \qCat _{r\infty }^{\protect \pbshape }$}{qCat}}{equation.4.19}{}}
\newlabel{complete:cor:terminal-cotensor}{{4.20}{20}{}{thm.4.20}{}}
\newlabel{complete:thm:stable}{{4.21}{20}{}{thm.4.21}{}}
\newlabel{complete:sec:algebras}{{5}{22}{Limits and colimits in the quasi-category of algebras}{section.5}{}}
\newlabel{complete:rec:algebras}{{5.1}{22}{homotopy coherent monads and their algebras}{thm.5.1}{}}
\newlabel{complete:obs:algcats-functoriality}{{5.2}{22}{}{thm.5.2}{}}
\newlabel{complete:eq:commutes-with-underlying}{{5.3}{23}{}{equation.5.3}{}}
\newlabel{complete:cor:monadic-colimits}{{5.5}{23}{}{thm.5.5}{}}
\newlabel{complete:cor:monadic-creates-u-split}{{5.6}{23}{}{thm.5.6}{}}
\newlabel{complete:thm:monadic-completeness}{{5.7}{23}{}{thm.5.7}{}}
\newlabel{complete:lem:W-.decomp}{{5.10}{25}{}{thm.5.10}{}}
\newlabel{complete:eq:projective-cell}{{5.11}{25}{Understanding the monadic forgetful functor}{equation.5.11}{}}
\newlabel{complete:cor:W-.decomp}{{5.12}{25}{}{thm.5.12}{}}
\newlabel{complete:eq:tower}{{5.13}{26}{Understanding the monadic forgetful functor}{equation.5.13}{}}
\newlabel{complete:eq:tower.step.pb}{{5.14}{26}{Understanding the monadic forgetful functor}{equation.5.14}{}}
\newlabel{complete:obs:W-.decomp.key}{{5.15}{26}{The key fact}{thm.5.15}{}}
\newlabel{complete:eq:terminal-fact}{{5.16}{26}{The key fact}{equation.5.16}{}}
\newlabel{complete:prop:monadic-terminal}{{5.17}{27}{}{thm.5.17}{}}
\newlabel{complete:eq:monadic-terminal}{{5.18}{27}{}{equation.5.18}{}}
\newlabel{complete:cor:monadic-terminal}{{5.20}{27}{}{thm.5.20}{}}
\newlabel{complete:eq:ind.step.filler.diag}{{5.21}{28}{Creation of terminal objects}{equation.5.21}{}}
\newlabel{complete:eq:lift1}{{5.22}{29}{Creation of limits}{equation.5.22}{}}
\newlabel{complete:thm:monadic-limit}{{5.24}{29}{}{thm.5.24}{}}
\newlabel{complete:eq:monadic-hypothesis}{{5.25}{29}{}{equation.5.25}{}}
\newlabel{complete:eq:monadic-conclusion}{{5.26}{29}{}{equation.5.26}{}}
\newlabel{complete:eq:pres-by-underlying}{{5.27}{30}{}{equation.5.27}{}}
\newlabel{complete:prop:monadic-limit-2}{{5.29}{30}{}{thm.5.29}{}}
\newlabel{complete:obs:expl-alg-desc}{{5.30}{30}{}{thm.5.30}{}}
\newlabel{complete:eq:expl-alg-desc}{{5.31}{30}{}{equation.5.31}{}}
\newlabel{complete:obs:W-.monad}{{5.32}{30}{}{thm.5.32}{}}
\newlabel{complete:eq:pre-commas}{{5.34}{31}{}{equation.5.34}{}}
\newlabel{complete:eq:squares-of-power}{{5.35}{32}{}{equation.5.35}{}}
\newlabel{complete:lem:technical-lem}{{5.36}{32}{}{thm.5.36}{}}
\newlabel{complete:tocindent-1}{0pt}
\newlabel{complete:tocindent0}{15.01021pt}
\newlabel{complete:tocindent1}{20.88377pt}
\newlabel{complete:tocindent2}{0pt}
\newlabel{complete:tocindent3}{0pt}


==> equipment_lab.tex <==
\newlabel{equipment:sec:background}{{2}{6}{Background}{section.2}{}}
\newlabel{equipment:ssec:cosmoi}{{2.1}{6}{\texorpdfstring {$\infty $}{infinity}-cosmoi and their homotopy 2-categories}{subsection.2.1}{}}
\newlabel{equipment:qcat.ctxt.cof.def}{{2.1.1}{6}{$\infty $-cosmos}{thm.2.1.1}{}}
\newlabel{equipment:qcat.ctxt.cof:a}{{{{(a)}}}{6}{$\infty $-cosmos}{Item.1}{}}
\newlabel{equipment:qcat.ctxt.cof:b}{{{{(b)}}}{6}{$\infty $-cosmos}{Item.2}{}}
\newlabel{equipment:qcat.ctxt.cof:c}{{{{(c)}}}{7}{$\infty $-cosmos}{Item.3}{}}
\newlabel{equipment:lem:triv.fib.stab}{{2.1.3}{7}{stability properties of trivial fibrations}{thm.2.1.3}{}}
\newlabel{equipment:itm:triv.fib.stab:a}{{{{(a)}}}{7}{stability properties of trivial fibrations}{Item.4}{}}
\newlabel{equipment:itm:triv.fib.stab:b}{{{{(b)}}}{7}{stability properties of trivial fibrations}{Item.5}{}}
\newlabel{equipment:itm:triv.fib.stab:c}{{{{(c)}}}{7}{stability properties of trivial fibrations}{Item.6}{}}
\newlabel{equipment:defn:closed-cosmoi}{{2.1.5}{7}{cartesian closed $\infty $-cosmoi}{thm.2.1.5}{}}
\newlabel{equipment:defn:sliced-cosmoi}{{2.1.6}{8}{sliced $\infty $-cosmoi}{thm.2.1.6}{}}
\newlabel{equipment:eq:sliced-map}{{2.1.7}{8}{sliced $\infty $-cosmoi}{equation.2.1.7}{}}
\newlabel{equipment:obs:general-functors-in-slices}{{2.1.8}{8}{}{thm.2.1.8}{}}
\newlabel{equipment:defn:qcat-ctxt-functor}{{2.1.9}{8}{}{thm.2.1.9}{}}
\newlabel{equipment:ex:functors}{{2.1.10}{9}{functors of $\infty $-cosmoi}{thm.2.1.10}{}}
\newlabel{equipment:prop:cartesian-closure}{{2.1.12}{10}{}{thm.2.1.12}{}}
\newlabel{equipment:defn:groupoidal-object}{{2.1.13}{10}{}{thm.2.1.13}{}}
\newlabel{equipment:ssec:sliced}{{2.2}{10}{Sliced homotopy 2-categories}{subsection.2.2}{}}
\newlabel{equipment:defn:two-slices}{{2.2.1}{10}{}{thm.2.2.1}{}}
\newlabel{equipment:prop:smothering-slice-comparison}{{2.2.2}{11}{}{thm.2.2.2}{}}
\newlabel{equipment:cor:slice-2-cat-comparison}{{2.2.3}{11}{}{thm.2.2.3}{}}
\newlabel{equipment:itm:slice-2-cat-comparison-equiv}{{{{(ii)}}}{11}{}{Item.10}{}}
\newlabel{equipment:itm:slice-2-cat-comparison-iso-class}{{{{(iii)}}}{12}{}{Item.11}{}}
\newlabel{equipment:itm:slice-2-cat-comparison-groupoidal}{{{{(iv)}}}{12}{}{Item.12}{}}
\newlabel{equipment:itm:slice-2-cat-comparison-adj}{{{{(v)}}}{12}{}{Item.13}{}}
\newlabel{equipment:rmk:adjunctions-pullback}{{2.2.6}{12}{}{thm.2.2.6}{}}
\newlabel{equipment:ssec:limits}{{2.3}{12}{Simplicial limits modeling comma \texorpdfstring {$\infty $}{infinity}-categories}{subsection.2.3}{}}
\newlabel{equipment:rec:comma}{{2.3.1}{13}{comma $\infty $-categories}{thm.2.3.1}{}}
\newlabel{equipment:eq:comma-as-simp-pullback}{{2.3.2}{13}{comma $\infty $-categories}{equation.2.3.2}{}}
\newlabel{equipment:eq:comma-square}{{2.3.3}{13}{comma $\infty $-categories}{equation.2.3.3}{}}
\newlabel{equipment:rec:ess.unique.1-cell.ind}{{2.3.4}{14}{}{thm.2.3.4}{}}
\newlabel{equipment:lem:equiv-invariance-of-commas}{{2.3.6}{14}{}{thm.2.3.6}{}}
\newlabel{equipment:lem:commas-pullback}{{2.3.7}{15}{}{thm.2.3.7}{}}
\newlabel{equipment:lem:equiv-to-comma}{{2.3.8}{15}{}{thm.2.3.8}{}}
\newlabel{equipment:ex:cone-comma-squares}{{2.3.9}{16}{}{thm.2.3.9}{}}
\newlabel{equipment:prop:induced-2-functor}{{2.3.10}{16}{}{thm.2.3.10}{}}
\newlabel{equipment:ssec:cartesian}{{2.4}{17}{Cartesian fibrations and groupoidal cartesian fibrations}{subsection.2.4}{}}
\newlabel{equipment:itm:weak.cart.i}{{{{(i)}}}{17}{cartesian 2-cells}{Item.17}{}}
\newlabel{equipment:itm:weak.cart.ii}{{{{(ii)}}}{17}{cartesian 2-cells}{Item.18}{}}
\newlabel{equipment:eq:2-cell.to.lift}{{2.4.3}{17}{cartesian fibration}{equation.2.4.3}{}}
\newlabel{equipment:itm:cart.fib.chars.i}{{{{(i)}}}{17}{}{Item.21}{}}
\newlabel{equipment:itm:cart.fib.chars.ii}{{{{(ii)}}}{18}{}{Item.22}{}}
\newlabel{equipment:itm:cart.fib.chars.iii}{{{{(iii)}}}{18}{}{Item.23}{}}
\newlabel{equipment:thm:gpd.cart.fib.chars}{{2.4.5}{18}{}{thm.2.4.5}{}}
\newlabel{equipment:itm:gpd.cart.fib.chars.i}{{{{(i)}}}{18}{}{Item.24}{}}
\newlabel{equipment:itm:gpd.cart.fib.chars.ii}{{{{(ii)}}}{18}{}{Item.25}{}}
\newlabel{equipment:itm:gpd.cart.fib.chars.iii}{{{{(iii)}}}{18}{}{Item.26}{}}
\newlabel{equipment:defn:cartesian-functor}{{2.4.7}{19}{}{thm.2.4.7}{}}
\newlabel{equipment:prop:cart-fib-pullback}{{2.4.8}{19}{\refIV {prop:cart-fib-pullback} and \refIV {cor:groupoidal-pullback}}{thm.2.4.8}{}}
\newlabel{equipment:sec:modules}{{3}{20}{Modules between \texorpdfstring {$\infty $}{infinity}-categories}{section.3}{}}
\newlabel{equipment:itm:cartesian-on-the-right}{{{{(i)}}}{20}{}{Item.29}{}}
\newlabel{equipment:itm:cocartesian-on-the-left}{{{{(ii)}}}{20}{}{Item.30}{}}
\newlabel{equipment:itm:groupoidal-fibers}{{{{(iii)}}}{20}{}{Item.31}{}}
\newlabel{equipment:lem:disc-cart-on-right}{{3.1.3}{20}{}{thm.3.1.3}{}}
\newlabel{equipment:prop:hom-is-a-module}{{3.1.4}{21}{}{thm.3.1.4}{}}
\newlabel{equipment:lem:sliced-adjunction-on-the-right}{{3.1.5}{22}{}{thm.3.1.5}{}}
\newlabel{equipment:itm:sliced-right-defn}{{{{(i)}}}{22}{}{Item.32}{}}
\newlabel{equipment:itm:sliced-right-fibred-adj}{{{{(ii)}}}{22}{}{Item.33}{}}
\newlabel{equipment:itm:sliced-right-adj}{{{{(iii)}}}{22}{}{Item.34}{}}
\newlabel{equipment:prop:two-sided-pullback}{{3.1.6}{23}{}{thm.3.1.6}{}}
\newlabel{equipment:cor:comma-is-a-module}{{3.1.7}{24}{}{thm.3.1.7}{}}
\newlabel{equipment:lem:two-sided-groupoidal-cells}{{3.1.9}{24}{}{thm.3.1.9}{}}
\newlabel{equipment:defn:horiz-comp}{{3.1.10}{25}{horizontal composition of isofibrations over products}{thm.3.1.10}{}}
\newlabel{equipment:lem:module-pullback-cartesian}{{3.1.12}{26}{}{thm.3.1.12}{}}
\newlabel{equipment:ex:modules-do-not-compose}{{3.1.13}{26}{}{thm.3.1.13}{}}
\newlabel{equipment:lem:span-maps-cartesian}{{3.2.1}{26}{}{thm.3.2.1}{}}
\newlabel{equipment:eq:span-map}{{3.2.2}{26}{}{equation.3.2.2}{}}
\newlabel{equipment:prop:two-sided-yoneda}{{3.2.4}{27}{}{thm.3.2.4}{}}
\newlabel{equipment:defn:1-cat-of-modules}{{3.2.5}{28}{}{thm.3.2.5}{}}
\newlabel{equipment:lem:full-yoneda}{{3.2.6}{28}{}{thm.3.2.6}{}}
\newlabel{equipment:defn:module-map}{{3.2.7}{29}{}{thm.3.2.7}{}}
\newlabel{equipment:lem:module-map-pullback-equivalence}{{3.2.8}{30}{}{thm.3.2.8}{}}
\newlabel{equipment:eq:pullback-for-UP}{{3.2.9}{30}{}{equation.3.2.9}{}}
\newlabel{equipment:lem:equiv-of-modules}{{3.3.1}{30}{}{thm.3.3.1}{}}
\newlabel{equipment:lem:rep-mod-char}{{3.3.2}{31}{}{thm.3.3.2}{}}
\newlabel{equipment:eq:r-equiv-defn}{{3.3.3}{31}{Equivalence of modules}{equation.3.3.3}{}}
\newlabel{equipment:eq:e-equiv-defn}{{3.3.4}{31}{Equivalence of modules}{equation.3.3.4}{}}
\newlabel{equipment:lem:qcat-pointwise-rep}{{3.3.5}{32}{}{thm.3.3.5}{}}
\newlabel{equipment:eq:lift-term-in-fibre}{{3.3.6}{32}{Equivalence of modules}{equation.3.3.6}{}}
\newlabel{equipment:cor:fibrewise-rep}{{3.3.7}{33}{}{thm.3.3.7}{}}
\newlabel{equipment:ex:adjoint-equivalence-mods}{{3.3.8}{33}{}{thm.3.3.8}{}}
\newlabel{equipment:sec:virtual}{{4}{34}{The virtual equipment of modules}{section.4}{}}
\newlabel{equipment:defn:double-iso-spans}{{4.1.1}{34}{the double category of isofibrations}{thm.4.1.1}{}}
\newlabel{equipment:eq:2-cell.bdary}{{4.1.2}{35}{the double category of isofibrations}{equation.4.1.2}{}}
\newlabel{equipment:eq:2-cell.hom.defn}{{4.1.3}{35}{the double category of isofibrations}{equation.4.1.3}{}}
\newlabel{equipment:obs:double-iso-spans}{{4.1.4}{35}{}{thm.4.1.4}{}}
\newlabel{equipment:eq:generic-cell}{{4.1.7}{36}{virtual double category}{equation.4.1.7}{}}
\newlabel{equipment:defn:modules-virtual}{{4.1.10}{38}{}{thm.4.1.10}{}}
\newlabel{equipment:defn:composable-modules}{{4.1.11}{38}{composable modules}{thm.4.1.11}{}}
\newlabel{equipment:obs:cells-above-a-comma}{{4.1.12}{38}{}{thm.4.1.12}{}}
\newlabel{equipment:eq:simplicial-pullback-of-module}{{4.2.1}{39}{The virtual equipment of modules}{equation.4.2.1}{}}
\newlabel{equipment:prop:cartesian-pullback-cells}{{4.2.2}{39}{}{thm.4.2.2}{}}
\newlabel{equipment:eq:cartesian-cell-UP}{{4.2.3}{39}{}{equation.4.2.3}{}}
\newlabel{equipment:prop:arrows-are-units}{{4.2.4}{40}{}{thm.4.2.4}{}}
\newlabel{equipment:defn:virtual-equipment}{{4.2.5}{41}{\cite [\S 7]{CruttwellShulman:2010au}}{thm.4.2.5}{}}
\newlabel{equipment:thm:virtual-equipment}{{4.2.6}{41}{}{thm.4.2.6}{}}
\newlabel{equipment:eq:multi-domain}{{4.3.3}{42}{composition of modules}{equation.4.3.3}{}}
\newlabel{equipment:eq:generic-composite}{{4.3.4}{42}{composition of modules}{equation.4.3.4}{}}
\newlabel{equipment:obs:unary-comp}{{4.3.5}{43}{nullary and unary composites}{thm.4.3.5}{}}
\newlabel{equipment:obs:comp-assoc}{{4.3.6}{43}{associativity of composition}{thm.4.3.6}{}}
\newlabel{equipment:obs:comp-cancel}{{4.3.7}{43}{left cancelation of composites}{thm.4.3.7}{}}
\newlabel{equipment:obs:comp-proof-strategy}{{4.3.8}{43}{}{thm.4.3.8}{}}
\newlabel{equipment:lem:comp-with-unit}{{4.3.9}{44}{composites with units}{thm.4.3.9}{}}
\newlabel{equipment:eq:comp-with-unit}{{4.3.10}{44}{composites with units}{equation.4.3.10}{}}
\newlabel{equipment:obs:comp-with-unit-over-comma}{{4.3.11}{44}{}{thm.4.3.11}{}}
\newlabel{equipment:defn:unit-cells}{{4.3.12}{44}{unit cells}{thm.4.3.12}{}}
\newlabel{equipment:lem:comp-with-unit-cells}{{4.3.13}{45}{composite with unit cells}{thm.4.3.13}{}}
\newlabel{equipment:defn:companion-conjoint}{{4.4.1}{46}{}{thm.4.4.1}{}}
\newlabel{equipment:thm:companion-conjoint}{{4.4.2}{47}{}{thm.4.4.2}{}}
\newlabel{equipment:cor:companion-conjoint}{{4.4.3}{49}{}{thm.4.4.3}{}}
\newlabel{equipment:lem:fibred-adjoint-reflection}{{4.4.4}{49}{}{thm.4.4.4}{}}
\newlabel{equipment:lem:one-sided-rep-comp}{{4.4.5}{49}{}{thm.4.4.5}{}}
\newlabel{equipment:cor:two-sided-rep-comp}{{4.4.7}{51}{}{thm.4.4.7}{}}
\newlabel{equipment:ex:comp-of-rep}{{4.4.8}{51}{}{thm.4.4.8}{}}
\newlabel{equipment:ex:two-sided-comma-as-composite}{{4.4.9}{51}{}{thm.4.4.9}{}}
\newlabel{equipment:lem:module-as-rep-composite}{{4.4.10}{51}{}{thm.4.4.10}{}}
\newlabel{equipment:lem:yoneda-embedding}{{4.4.11}{52}{}{thm.4.4.11}{}}
\newlabel{equipment:rmk:yoneda-embedding}{{4.4.12}{53}{}{thm.4.4.12}{}}
\newlabel{equipment:sec:pointwise-kan}{{5}{53}{Pointwise Kan extensions}{section.5}{}}
\newlabel{equipment:ssec:exact-squares}{{5.1}{53}{Exact squares}{subsection.5.1}{}}
\newlabel{equipment:defn:exact-square}{{5.1.1}{53}{exact squares}{thm.5.1.1}{}}
\newlabel{equipment:lem:exact-squares-comp}{{5.1.2}{54}{composites of exact squares}{thm.5.1.2}{}}
\newlabel{equipment:lem:comma-exact}{{5.1.3}{55}{}{thm.5.1.3}{}}
\newlabel{equipment:lem:pullback-exact}{{5.1.4}{55}{}{thm.5.1.4}{}}
\newlabel{equipment:lem:product-exact-square}{{5.1.5}{56}{}{thm.5.1.5}{}}
\newlabel{equipment:lem:product-comma-exact}{{5.1.6}{57}{}{thm.5.1.6}{}}
\newlabel{equipment:ssec:pointwise-kan}{{5.2}{58}{Pointwise Kan Extensions}{subsection.5.2}{}}
\newlabel{equipment:defn:right-extension-mod}{{5.2.1}{58}{right extension of modules}{thm.5.2.1}{}}
\newlabel{equipment:lem:mod-extensions-in-2-cat}{{5.2.2}{58}{}{thm.5.2.2}{}}
\newlabel{equipment:prop:pointwise-kan}{{5.2.4}{59}{}{thm.5.2.4}{}}
\newlabel{equipment:eq:pointwise-right-extension}{{5.2.5}{59}{}{equation.5.2.5}{}}
\newlabel{equipment:itm:pointwise-exact-stable}{{{{(i)}}}{59}{}{Item.40}{}}
\newlabel{equipment:itm:pointwise-comma-stable}{{{{(ii)}}}{59}{}{Item.41}{}}
\newlabel{equipment:itm:pointwise-in-mod}{{{{(iii)}}}{59}{}{Item.42}{}}
\newlabel{equipment:itm:pointwise-exact-stable-in-mod}{{{{(iv)}}}{59}{}{Item.43}{}}
\newlabel{equipment:defn:fully-faithful}{{5.2.7}{61}{fully faithful}{thm.5.2.7}{}}
\newlabel{equipment:ssec:pointwise-kan-closed}{{5.3}{62}{Pointwise Kan extensions in a cartesian closed \texorpdfstring {$\infty $}{infinity}-cosmos}{subsection.5.3}{}}
\newlabel{equipment:prop:ran-abs-lifting}{{5.3.1}{63}{}{thm.5.3.1}{}}
\newlabel{equipment:eq:pointwise-kan-abs-lifting}{{5.3.2}{63}{}{equation.5.3.2}{}}
\newlabel{equipment:eq:limit-abs-lifting}{{5.3.3}{64}{Pointwise Kan extensions in a cartesian closed \texorpdfstring {$\infty $}{infinity}-cosmos}{equation.5.3.3}{}}
\newlabel{equipment:prop:limits-as-pointwise-kan}{{5.3.4}{64}{}{thm.5.3.4}{}}
\newlabel{equipment:defn:initial-final}{{5.3.5}{64}{initial/final functor}{thm.5.3.5}{}}
\newlabel{equipment:prop:beck-chevalley}{{5.3.9}{66}{Beck-Chevalley condition}{thm.5.3.9}{}}
\newlabel{equipment:rmk:qcat-derivator}{{5.3.10}{67}{on derivators for (co)complete quasi-categories}{thm.5.3.10}{}}
\newlabel{equipment:eq:qcat-derivator}{{5.3.11}{68}{on derivators for (co)complete quasi-categories}{equation.5.3.11}{}}
\newlabel{equipment:eq:mod-right-ext}{{5.3.12}{69}{on derivators for (co)complete quasi-categories}{equation.5.3.12}{}}
\newlabel{equipment:tocindent-1}{0pt}
\newlabel{equipment:tocindent0}{15.01021pt}
\newlabel{equipment:tocindent1}{20.88377pt}
\newlabel{equipment:tocindent2}{34.49158pt}
\newlabel{equipment:tocindent3}{0pt}


==> foundations_lab.tex <==
\newlabel{found:sec:background}{{2}{6}{Background on quasi-categories}{section.2}{}}
\newlabel{found:obs:size-conventions}{{2.0.1}{6}{size}{thm.2.0.1}{}}
\newlabel{found:subsect:simplicial.notation}{{2.1}{6}{Some standard simplicial notation}{subsection.2.1}{}}
\newlabel{found:ntn:simp.op}{{2.1.1}{6}{simplicial operators}{thm.2.1.1}{}}
\newlabel{found:ntn:simplicial-sets}{{2.1.2}{6}{(augmented) simplicial sets}{thm.2.1.2}{}}
\newlabel{found:rec:augmentation}{{2.1.3}{7}{augmentation}{thm.2.1.3}{}}
\newlabel{found:ntn:faces-by-vertices}{{2.1.5}{8}{faces of \protect {$\Del ^n$}}{thm.2.1.5}{}}
\newlabel{found:ntn:simplicial-hom-space}{{2.1.6}{8}{internal hom}{thm.2.1.6}{}}
\newlabel{found:rec:hty-category}{{2.2.2}{8}{the homotopy category}{thm.2.2.2}{}}
\newlabel{found:eq:homotopy-of-1-simplices}{{2.2.3}{9}{the homotopy category}{equation.2.2.3}{}}
\newlabel{found:rec:qmc-quasicat}{{2.2.5}{9}{the model category of quasi-categories}{thm.2.2.5}{}}
\newlabel{found:rec:leibniz}{{2.2.6}{9}{Leibniz constructions}{thm.2.2.6}{}}
\newlabel{found:rec:cart-modcat}{{2.2.8}{10}{cartesian model categories}{thm.2.2.8}{}}
\newlabel{found:obs:isofibration-closure}{{2.2.9}{10}{closure properties of isofibrations}{thm.2.2.9}{}}
\newlabel{found:defn:equivalences}{{2.3.1}{10}{isomorphisms in quasi-categories}{thm.2.3.1}{}}
\newlabel{found:rec:marked-prod-exp}{{2.3.4}{11}{products and exponentiation}{thm.2.3.4}{}}
\newlabel{found:rmk:equiv-markings}{{2.3.5}{12}{isomorphisms and markings}{thm.2.3.5}{}}
\newlabel{found:prop:joyal-special-horn}{{2.3.7}{12}{Joyal}{thm.2.3.7}{}}
\newlabel{found:rec:qmc-quasi-marked}{{2.3.8}{12}{the model structure of naturally marked quasi-categories}{thm.2.3.8}{}}
\newlabel{found:obs:nat-mark-homs}{{2.3.9}{13}{natural markings, internal homs, and products}{thm.2.3.9}{}}
\newlabel{found:lem:pointwise-equiv}{{2.3.10}{13}{pointwise isomorphisms are isomorphisms}{thm.2.3.10}{}}
\newlabel{found:eq:pointwise-equivalence-square}{{2.3.11}{13}{Isomorphisms and marked simplicial sets}{equation.2.3.11}{}}
\newlabel{found:cor:pointwise-equiv}{{2.3.12}{14}{}{thm.2.3.12}{}}
\newlabel{found:obs:marked-arrow-subcat}{{2.3.13}{14}{}{thm.2.3.13}{}}
\newlabel{found:subsec:join}{{2.4}{14}{Join and slice}{subsection.2.4}{}}
\newlabel{found:defn:join-dec}{{2.4.1}{15}{joins and d{\'e}calage}{thm.2.4.1}{}}
\newlabel{found:defn:slices}{{2.4.2}{15}{d{\'e}calage and slices}{thm.2.4.2}{}}
\newlabel{found:obs:slice-and-qcats}{{2.4.3}{16}{slices of quasi-categories}{thm.2.4.3}{}}
\newlabel{found:def:fat-join}{{2.4.4}{16}{fat join}{thm.2.4.4}{}}
\newlabel{found:eq:fat-join-def}{{2.4.5}{16}{fat join}{equation.2.4.5}{}}
\newlabel{found:eq:fat-join-cong}{{2.4.6}{17}{fat join}{equation.2.4.6}{}}
\newlabel{found:defn:fat-slices}{{2.4.7}{17}{fat slice}{thm.2.4.7}{}}
\newlabel{found:eq:join-comp-def}{{2.4.9}{17}{comparing join constructions}{equation.2.4.9}{}}
\newlabel{found:eq:tnm-def}{{2.4.10}{17}{comparing join constructions}{equation.2.4.10}{}}
\newlabel{found:prop:join-fatjoin-equiv}{{2.4.11}{18}{}{thm.2.4.11}{}}
\newlabel{found:lem:slices-quillen}{{2.4.12}{18}{}{thm.2.4.12}{}}
\newlabel{found:prop:slice-fatslice-equiv}{{2.4.13}{18}{slices and fat slices of a quasi-category are equivalent}{thm.2.4.13}{}}
\newlabel{found:rmk:map-slices}{{2.4.14}{19}{}{thm.2.4.14}{}}
\newlabel{found:sec:twocat}{{3}{19}{The 2-category of quasi-categories}{section.3}{}}
\newlabel{found:obs:simp-to-2-cats}{{3.1.2}{20}{}{thm.3.1.2}{}}
\newlabel{found:def:qCat-2}{{3.2.1}{21}{the 2-category of quasi-categories}{thm.3.2.1}{}}
\newlabel{found:eq:qCat2homdefn}{{3.2.2}{21}{the 2-category of quasi-categories}{equation.3.2.2}{}}
\newlabel{found:obs:pointwise-iso-reprise}{{3.2.3}{22}{pointwise isomorphisms are isomorphisms (reprise)}{thm.3.2.3}{}}
\newlabel{found:prop:qcat2closed}{{3.2.4}{22}{}{thm.3.2.4}{}}
\newlabel{found:defn:2-cat.of.all.simpsets}{{3.2.5}{23}{the 2-category of all simplicial sets}{thm.3.2.5}{}}
\newlabel{found:rmk:exp2functor}{{3.2.6}{23}{}{thm.3.2.6}{}}
\newlabel{found:lem:2-cat.equivs}{{3.2.8}{23}{}{thm.3.2.8}{}}
\newlabel{found:prop:equivsareequivs}{{3.2.9}{24}{}{thm.3.2.9}{}}
\newlabel{found:prop:equivsareequivs2}{{3.2.10}{24}{}{thm.3.2.10}{}}
\newlabel{found:subsec:weak-2-limits}{{3.3}{24}{Weak 2-limits}{subsection.3.3}{}}
\newlabel{found:defn:smothering}{{3.3.1}{24}{smothering functors}{thm.3.3.1}{}}
\newlabel{found:lem:smothering}{{3.3.2}{25}{fibres of smothering functors}{thm.3.3.2}{}}
\newlabel{found:defn:weak2limit}{{3.3.3}{25}{weak 2-limits in a 2-category}{thm.3.3.3}{}}
\newlabel{found:eq:cone-induced}{{3.3.4}{25}{weak 2-limits in a 2-category}{equation.3.3.4}{}}
\newlabel{found:lem:unique-weak-2-limits}{{3.3.5}{25}{}{thm.3.3.5}{}}
\newlabel{found:lem:weak-simplification}{{3.3.6}{26}{}{thm.3.3.6}{}}
\newlabel{found:eq:qCat.wl.comp.1}{{3.3.7}{26}{Weak 2-limits}{equation.3.3.7}{}}
\newlabel{found:prop:weak-cotensors}{{3.3.9}{27}{}{thm.3.3.9}{}}
\newlabel{found:eq:arrowinhA}{{3.3.10}{27}{Weak 2-limits}{equation.3.3.10}{}}
\newlabel{found:eq:liftedarrowinA2}{{3.3.11}{28}{Weak 2-limits}{equation.3.3.11}{}}
\newlabel{found:prop:weak-iso-cotensor}{{3.3.13}{28}{}{thm.3.3.13}{}}
\newlabel{found:prop:weak-homotopy-pullbacks}{{3.3.14}{29}{}{thm.3.3.14}{}}
\newlabel{found:def:comma-obj}{{3.3.15}{30}{comma objects}{thm.3.3.15}{}}
\newlabel{found:lem:comma-obj}{{3.3.16}{30}{}{thm.3.3.16}{}}
\newlabel{found:lem:comma-obj-maps}{{3.3.17}{30}{maps induced between comma objects}{thm.3.3.17}{}}
\newlabel{found:prop:weakcomma}{{3.3.18}{31}{}{thm.3.3.18}{}}
\newlabel{found:eq:commacat-comp}{{3.3.19}{31}{Weak 2-limits}{equation.3.3.19}{}}
\newlabel{found:obs:unpacking-weak-comma-objects}{{3.3.20}{31}{unpacking the universal property of weak comma objects}{thm.3.3.20}{}}
\newlabel{found:eq:weak-comma-prop}{{3.3.21}{31}{unpacking the universal property of weak comma objects}{equation.3.3.21}{}}
\newlabel{found:eq:standard-comma-pic}{{3.3.22}{32}{unpacking the universal property of weak comma objects}{equation.3.3.22}{}}
\newlabel{found:eq:comma-cone}{{3.3.23}{32}{unpacking the universal property of weak comma objects}{equation.3.3.23}{}}
\newlabel{found:eq:comma-ind-1cell-prop}{{3.3.24}{32}{unpacking the universal property of weak comma objects}{equation.3.3.24}{}}
\newlabel{found:eq:comma-ind-2cell-data}{{3.3.25}{32}{unpacking the universal property of weak comma objects}{equation.3.3.25}{}}
\newlabel{found:eq:comma-ind-2cell-compat}{{3.3.26}{33}{unpacking the universal property of weak comma objects}{equation.3.3.26}{}}
\newlabel{found:lem:1cell-ind-uniqueness}{{3.3.27}{33}{1-cell induction is unique up to isomorphism}{thm.3.3.27}{}}
\newlabel{found:subsec:slice-2cats-of-qcats}{{3.4}{33}{Slices of the category of quasi-categories}{subsection.3.4}{}}
\newlabel{found:defn:enriched-slice}{{3.4.1}{33}{enriching the slices of $\qCat $}{thm.3.4.1}{}}
\newlabel{found:eq:slice-hom-objects}{{3.4.2}{34}{enriching the slices of $\qCat $}{equation.3.4.2}{}}
\newlabel{found:obs:fibred-pushforward}{{3.4.3}{34}{pushforward}{thm.3.4.3}{}}
\newlabel{found:obs:fibred-pullback}{{3.4.4}{34}{pullback}{thm.3.4.4}{}}
\newlabel{found:defn:smothering-2-functor}{{3.4.6}{35}{smothering 2-functor}{thm.3.4.6}{}}
\newlabel{found:prop:slice-smothering-2-functor}{{3.4.7}{35}{}{thm.3.4.7}{}}
\newlabel{found:defn:representable-isofibrations}{{3.4.8}{35}{representably defined isofibrations in 2-categories}{thm.3.4.8}{}}
\newlabel{found:lem:representable-isofibration}{{3.4.9}{36}{}{thm.3.4.9}{}}
\newlabel{found:lem:proj-is-1-conservative}{{3.4.10}{36}{}{thm.3.4.10}{}}
\newlabel{found:eq:equiv-to-lift}{{3.4.11}{36}{}{equation.3.4.11}{}}
\newlabel{found:cor:recog-fibred-equivs}{{3.4.12}{36}{}{thm.3.4.12}{}}
\newlabel{found:defn:fibred-equivalence}{{3.4.13}{37}{fibred equivalence}{thm.3.4.13}{}}
\newlabel{found:obs:1cell-ind-uniqueness-reloaded}{{3.5.1}{37}{uniqueness of 1-cell induction revisited}{thm.3.5.1}{}}
\newlabel{found:eq:induced-1-cell-comparison}{{3.5.2}{37}{uniqueness of 1-cell induction revisited}{equation.3.5.2}{}}
\newlabel{found:obs:squares-set}{{3.5.3}{38}{}{thm.3.5.3}{}}
\newlabel{found:obs:groupoid-components}{{3.5.4}{38}{}{thm.3.5.4}{}}
\newlabel{found:lem:sq-as-a-functor}{{3.5.5}{38}{}{thm.3.5.5}{}}
\newlabel{found:eq:the-real-sq-functor}{{3.5.6}{38}{}{equation.3.5.6}{}}
\newlabel{found:lem:cpts-and-comma-2-cells}{{3.5.7}{39}{}{thm.3.5.7}{}}
\newlabel{found:eq:first-comma-cone}{{3.5.8}{39}{}{equation.3.5.8}{}}
\newlabel{found:eq:other-comma-cone}{{3.5.9}{39}{}{equation.3.5.9}{}}
\newlabel{found:sec:qcatadj}{{4}{40}{Adjunctions of quasi-categories}{section.4}{}}
\newlabel{found:defn:adjunction}{{4.0.1}{40}{adjunction}{thm.4.0.1}{}}
\newlabel{found:ex:simp.quillen.adj}{{4.0.4}{41}{}{thm.4.0.4}{}}
\newlabel{found:subsec:RARI}{{4.1}{42}{Right adjoint right inverse adjunctions}{subsection.4.1}{}}
\newlabel{found:defn:RARI}{{4.1.1}{42}{}{thm.4.1.1}{}}
\newlabel{found:lem:adjunction.from.isos}{{4.1.2}{42}{}{thm.4.1.2}{}}
\newlabel{found:eq:triangle-calculation-1}{{4.1.3}{42}{Right adjoint right inverse adjunctions}{equation.4.1.3}{}}
\newlabel{found:eq:triangle-calculation-2}{{4.1.4}{43}{Right adjoint right inverse adjunctions}{equation.4.1.4}{}}
\newlabel{found:rmk:idempotent-isomorphisms}{{4.1.5}{43}{idempotent isomorphisms}{thm.4.1.5}{}}
\newlabel{found:lem:technicalsliceadjunction}{{4.1.6}{43}{}{thm.4.1.6}{}}
\newlabel{found:eq:technicalsliceadjunction}{{4.1.7}{43}{}{equation.4.1.7}{}}
\newlabel{found:lem:isofibration-RARI}{{4.1.8}{44}{}{thm.4.1.8}{}}
\newlabel{found:subsec:terminal}{{4.2}{44}{Terminal objects as adjoint functors}{subsection.4.2}{}}
\newlabel{found:defn:terminal}{{4.2.1}{44}{terminal objects}{thm.4.2.1}{}}
\newlabel{found:ex:slice-terminal}{{4.2.2}{45}{slices have terminal objects}{thm.4.2.2}{}}
\newlabel{found:lem:min-term-pres}{{4.2.3}{45}{minimal information required to display a terminal object}{thm.4.2.3}{}}
\newlabel{found:lem:adj-ext-univ}{{4.2.4}{45}{}{thm.4.2.4}{}}
\newlabel{found:prop:terminal-ext-univ}{{4.2.5}{46}{}{thm.4.2.5}{}}
\newlabel{found:ex:terminaldefn}{{4.2.6}{46}{}{thm.4.2.6}{}}
\newlabel{found:prop:adj-comp}{{4.3.1}{47}{}{thm.4.3.1}{}}
\newlabel{found:prop:equivtoadjoint}{{4.3.2}{47}{}{thm.4.3.2}{}}
\newlabel{found:prop:expadj}{{4.3.3}{47}{}{thm.4.3.3}{}}
\newlabel{found:prop:terminaldefn}{{4.3.4}{48}{}{thm.4.3.4}{}}
\newlabel{found:eq:commaobjdefn}{{4.4.1}{48}{The universal property of adjunctions}{equation.4.4.1}{}}
\newlabel{found:prop:adjointequiv}{{4.4.2}{48}{}{thm.4.4.2}{}}
\newlabel{found:prop:adjointequivconverse}{{4.4.3}{49}{}{thm.4.4.3}{}}
\newlabel{found:obs:pointwise-adjoint-correspondence}{{4.4.4}{50}{the hom-spaces of a quasi-category}{thm.4.4.4}{}}
\newlabel{found:rmk:vs-lurie-adjunction}{{4.4.5}{50}{}{thm.4.4.5}{}}
\newlabel{found:lem:slice-equiv-comma}{{4.4.6}{50}{}{thm.4.4.6}{}}
\newlabel{found:prop:terminalconverse}{{4.4.7}{51}{}{thm.4.4.7}{}}
\newlabel{found:prop:pointwise-univ-adj}{{4.4.8}{51}{the pointwise universal property of an adjunction}{thm.4.4.8}{}}
\newlabel{found:obs:universal-property-of-epsilon}{{4.4.10}{52}{unpacking this pointwise universal property of an adjunction}{thm.4.4.10}{}}
\newlabel{found:lem:RARI-lifting}{{4.4.12}{53}{right adjoint right inverse as a lifting property}{thm.4.4.12}{}}
\newlabel{found:eq:RARI-lifting}{{4.4.13}{53}{right adjoint right inverse as a lifting property}{equation.4.4.13}{}}
\newlabel{found:subsec:fibred.adjunction}{{4.5}{54}{Fibred adjunctions}{subsection.4.5}{}}
\newlabel{found:defn:fibred.adj}{{4.5.1}{54}{fibred adjunctions}{thm.4.5.1}{}}
\newlabel{found:lem:missed-lemma}{{4.5.2}{55}{}{thm.4.5.2}{}}
\newlabel{found:cor:missed-lemma}{{4.5.3}{55}{}{thm.4.5.3}{}}
\newlabel{found:ex:fibred-technical-slice-adjunction}{{4.5.4}{55}{}{thm.4.5.4}{}}
\newlabel{found:ex:isofib-section.fibred.adjunction}{{4.5.5}{55}{fibred isofibration RARIs}{thm.4.5.5}{}}
\newlabel{found:eq:fibred.terminal}{{4.5.6}{55}{fibred isofibration RARIs}{equation.4.5.6}{}}
\newlabel{found:obs:isofib-section.fibred.adjunction}{{4.5.7}{56}{}{thm.4.5.7}{}}
\newlabel{found:ex:comp.ident.adj}{{4.5.8}{56}{}{thm.4.5.8}{}}
\newlabel{found:eq:comp.ident.adj}{{4.5.9}{57}{}{equation.4.5.9}{}}
\newlabel{found:sec:limits}{{5}{57}{Limits and colimits}{section.5}{}}
\newlabel{found:defn:abs-right-lift}{{5.0.1}{57}{}{thm.5.0.1}{}}
\newlabel{found:eq:absRlifting}{{5.0.2}{57}{}{equation.5.0.2}{}}
\newlabel{found:eq:abs-lifting-property}{{5.0.3}{57}{}{equation.5.0.3}{}}
\newlabel{found:ex:adjasabslifting}{{5.0.4}{58}{}{thm.5.0.4}{}}
\newlabel{found:eq:adjasabslifting}{{5.0.5}{58}{}{equation.5.0.5}{}}
\newlabel{found:eq:unitdefn}{{5.0.6}{58}{Limits and colimits}{equation.5.0.6}{}}
\newlabel{found:eq:comma-cones}{{5.1.1}{58}{Absolute liftings and comma objects}{equation.5.1.1}{}}
\newlabel{found:eq:w-def-prop}{{5.1.2}{59}{Absolute liftings and comma objects}{equation.5.1.2}{}}
\newlabel{found:prop:absliftingtranslation}{{5.1.3}{59}{}{thm.5.1.3}{}}
\newlabel{found:eq:induced-u-from-nattrans-k}{{5.1.4}{60}{Absolute liftings and comma objects}{equation.5.1.4}{}}
\newlabel{found:lem:represented-nat-trans}{{5.1.6}{60}{}{thm.5.1.6}{}}
\newlabel{found:eq:rel-mu-lambda}{{5.1.7}{61}{Absolute liftings and comma objects}{equation.5.1.7}{}}
\newlabel{found:prop:absliftingtranslation2}{{5.1.8}{61}{}{thm.5.1.8}{}}
\newlabel{found:eq:absRlifting.2}{{5.1.9}{62}{}{equation.5.1.9}{}}
\newlabel{found:eq:induced-from-lambda}{{5.1.10}{62}{}{equation.5.1.10}{}}
\newlabel{found:eq:t-for-lim-def-prop}{{5.1.11}{63}{Absolute liftings and comma objects}{equation.5.1.11}{}}
\newlabel{found:prop:right.liftings.as.fibred.terminal.objects}{{5.1.12}{63}{}{thm.5.1.12}{}}
\newlabel{found:eq:fibred.terminal.2}{{5.1.13}{63}{}{equation.5.1.13}{}}
\newlabel{found:eq:limit-lifting-prop}{{5.1.14}{63}{Absolute liftings and comma objects}{equation.5.1.14}{}}
\newlabel{found:eq:m-def-prop}{{5.1.15}{64}{Absolute liftings and comma objects}{equation.5.1.15}{}}
\newlabel{found:obs:right.liftings.as.fibred.terminal.objects}{{5.1.16}{64}{}{thm.5.1.16}{}}
\newlabel{found:prop:translated.lifting}{{5.1.17}{64}{}{thm.5.1.17}{}}
\newlabel{found:eq:orig.lifting}{{5.1.18}{64}{}{equation.5.1.18}{}}
\newlabel{found:eq:translated.lifting}{{5.1.19}{64}{}{equation.5.1.19}{}}
\newlabel{found:eq:ran.as.fibred.adj}{{5.1.20}{65}{Absolute liftings and comma objects}{equation.5.1.20}{}}
\newlabel{found:eq:adj.for.trans}{{5.1.21}{65}{Absolute liftings and comma objects}{equation.5.1.21}{}}
\newlabel{found:defn:limit}{{5.2.2}{66}{}{thm.5.2.2}{}}
\newlabel{found:eq:genericlimit}{{5.2.3}{66}{}{equation.5.2.3}{}}
\newlabel{found:eq:genericcolimit}{{5.2.4}{66}{}{equation.5.2.4}{}}
\newlabel{found:prop:limits.as.terminal.objects}{{5.2.6}{67}{}{thm.5.2.6}{}}
\newlabel{found:lem:cone-equiv-fatcone}{{5.2.7}{67}{}{thm.5.2.7}{}}
\newlabel{found:prop:limits.are.limits}{{5.2.8}{68}{}{thm.5.2.8}{}}
\newlabel{found:defn:families.of.diagrams}{{5.2.9}{68}{}{thm.5.2.9}{}}
\newlabel{found:eq:limits.of.a.family}{{5.2.10}{68}{}{equation.5.2.10}{}}
\newlabel{found:prop:families.of.diagrams}{{5.2.11}{68}{}{thm.5.2.11}{}}
\newlabel{found:prop:limitsasadjunctions}{{5.2.12}{69}{}{thm.5.2.12}{}}
\newlabel{found:prop:RAPL}{{5.2.13}{69}{}{thm.5.2.13}{}}
\newlabel{found:cor:equivprescolim}{{5.2.14}{70}{}{thm.5.2.14}{}}
\newlabel{found:obs:transpose-abs-lifting}{{5.2.15}{70}{}{thm.5.2.15}{}}
\newlabel{found:eq:untransposed}{{5.2.16}{70}{}{equation.5.2.16}{}}
\newlabel{found:eq:transposed}{{5.2.17}{70}{}{equation.5.2.17}{}}
\newlabel{found:prop:pointwise-limits-in-functor-quasi-categories}{{5.2.18}{71}{pointwise limits in functor quasi-categories}{thm.5.2.18}{}}
\newlabel{found:prop:ran.adj.limits}{{5.2.19}{71}{}{thm.5.2.19}{}}
\newlabel{found:cor:ran.adj.limits}{{5.2.20}{72}{}{thm.5.2.20}{}}
\newlabel{found:ntn:pb.po.joins}{{5.2.22}{73}{pushout and pullback diagrams}{thm.5.2.22}{}}
\newlabel{found:obs:loops.diag.fam}{{5.2.24}{73}{}{thm.5.2.24}{}}
\newlabel{found:defn:loop.susp}{{5.2.25}{73}{loop spaces and suspensions}{thm.5.2.25}{}}
\newlabel{found:prop:loops-suspension}{{5.2.27}{74}{}{thm.5.2.27}{}}
\newlabel{found:eq:pullback.pushout.adj}{{5.2.28}{74}{Limits and colimits as absolute lifting diagrams}{equation.5.2.28}{}}
\newlabel{found:eq:loop.susp.var}{{5.2.29}{74}{Limits and colimits as absolute lifting diagrams}{equation.5.2.29}{}}
\newlabel{found:thm:splitgeorealizations}{{5.3.1}{76}{}{thm.5.3.1}{}}
\newlabel{found:lem:doms2catlemma}{{5.3.2}{76}{}{thm.5.3.2}{}}
\newlabel{found:sec:pointwise}{{6}{78}{Pointwise universal properties}{section.6}{}}
\newlabel{found:defn:pointwise-abs-lifting}{{6.1.1}{78}{pointwise universal property of absoluting lifting diagrams}{thm.6.1.1}{}}
\newlabel{found:eq:pointwise-absRlifting}{{6.1.2}{78}{pointwise universal property of absoluting lifting diagrams}{equation.6.1.2}{}}
\newlabel{found:lem:pointwise-terminal}{{6.1.3}{78}{}{thm.6.1.3}{}}
\newlabel{found:thm:pointwise}{{6.1.4}{79}{}{thm.6.1.4}{}}
\newlabel{found:eq:term.obj.assumption}{{6.1.5}{79}{Pointwise absolute lifting}{equation.6.1.5}{}}
\newlabel{found:eq:term.obj.extension}{{6.1.6}{79}{Pointwise absolute lifting}{equation.6.1.6}{}}
\newlabel{found:eq:term.obj.lifting}{{6.1.7}{79}{Pointwise absolute lifting}{equation.6.1.7}{}}
\newlabel{found:cor:pointwise}{{6.1.8}{80}{}{thm.6.1.8}{}}
\newlabel{found:thm:simplicial-Quillen-adjunction}{{6.2.1}{81}{}{thm.6.2.1}{}}
\newlabel{found:eq:simp.adj.extension}{{6.2.2}{82}{Simplicial Quillen adjunctions are adjunctions of quasi-categories}{equation.6.2.2}{}}
\newlabel{found:tocindent-1}{0pt}
\newlabel{found:tocindent0}{15.01021pt}
\newlabel{found:tocindent1}{20.88377pt}
\newlabel{found:tocindent2}{34.49158pt}
\newlabel{found:tocindent3}{0pt}


==> reedy_lab.tex <==
\newlabel{reedy:eq:reedy's.po}{{1.1}{2}{Introduction}{equation.1.1}{}}
\newlabel{reedy:eq:reedy's.delta}{{1.2}{3}{Introduction}{equation.1.2}{}}
\newlabel{reedy:ntn:index-stuff}{{1.4}{4}{general index notation}{thm.1.4}{}}
\newlabel{reedy:ex:tensor-cotensor}{{1.6}{5}{tensors and cotensors}{thm.1.6}{}}
\newlabel{reedy:defn:ends-and-coends}{{1.7}{6}{ends and coends}{thm.1.7}{}}
\newlabel{reedy:defn:cat-of-elts}{{1.8}{6}{categories of elements}{thm.1.8}{}}
\newlabel{reedy:obs:coend-in-sets}{{1.9}{7}{coends in sets}{thm.1.9}{}}
\newlabel{reedy:eq:pb-coends-in-sets}{{1.10}{7}{coends in sets}{equation.1.10}{}}
\newlabel{reedy:eq:wlimformula}{{1.12}{7}{weighted limits and colimits}{equation.1.12}{}}
\newlabel{reedy:ex:weighted-conical}{{1.13}{7}{terminal weights}{thm.1.13}{}}
\newlabel{reedy:ex:weighted-yoneda}{{1.14}{8}{representable weights}{thm.1.14}{}}
\newlabel{reedy:eq:yoneda}{{1.15}{8}{representable weights}{equation.1.15}{}}
\newlabel{reedy:ex:matching.preview}{{1.17}{8}{}{thm.1.17}{}}
\newlabel{reedy:obs:weighted.as.ordinary}{{1.19}{8}{weighted limits as ordinary limits}{thm.1.19}{}}
\newlabel{reedy:obs:wcolim-in-sets}{{1.21}{8}{weighted colimits in sets}{thm.1.21}{}}
\newlabel{reedy:sec:reedy}{{2}{9}{Reedy categories}{section.2}{}}
\newlabel{reedy:defn:reedy}{{2.1}{9}{Reedy categories}{thm.2.1}{}}
\newlabel{reedy:ex:poset.reedy}{{2.3}{9}{finite posets}{thm.2.3}{}}
\newlabel{reedy:ex:pushout.reedy.alt}{{2.4}{9}{the pushout diagram}{thm.2.4}{}}
\newlabel{reedy:ex:parallel.pair.reedy}{{2.5}{10}{the parallel pair}{thm.2.5}{}}
\newlabel{reedy:defn:factorisations}{{2.8}{10}{categories of factorisations}{thm.2.8}{}}
\newlabel{reedy:lem:reedy-fact-connect}{{2.9}{10}{}{thm.2.9}{}}
\newlabel{reedy:sec:latching}{{3}{11}{Latching and matching objects}{section.3}{}}
\newlabel{reedy:rec:skel-coskel}{{3.1}{11}{skeleta and coskeleta}{thm.3.1}{}}
\newlabel{reedy:eq:4}{{3.2}{12}{skeleta and coskeleta}{equation.3.2}{}}
\newlabel{reedy:obs:skel-colim}{{3.3}{12}{}{thm.3.3}{}}
\newlabel{reedy:eq:5}{{3.4}{12}{}{equation.3.4}{}}
\newlabel{reedy:lem:skeleta-colimit}{{3.5}{13}{}{thm.3.5}{}}
\newlabel{reedy:eq:6}{{3.6}{13}{}{equation.3.6}{}}
\newlabel{reedy:obs:skel-reps}{{3.7}{13}{skeleta of representables and factorisations}{thm.3.7}{}}
\newlabel{reedy:eq:sk-rep-coend}{{3.8}{13}{skeleta of representables and factorisations}{equation.3.8}{}}
\newlabel{reedy:lem:inductive.defn}{{3.10}{15}{inductive definition of diagrams}{thm.3.10}{}}
\newlabel{reedy:obs:inductive.defn}{{3.11}{15}{inductive definition of natural transformations}{thm.3.11}{}}
\newlabel{reedy:ex:sequence-induction}{{3.12}{15}{}{thm.3.12}{}}
\newlabel{reedy:defn:latching}{{3.13}{16}{latching and matching objects}{thm.3.13}{}}
\newlabel{reedy:ex:simp-latching-1}{{3.14}{16}{}{thm.3.14}{}}
\newlabel{reedy:obs:weights-latching}{{3.15}{16}{weights for latching and matching objects}{thm.3.15}{}}
\newlabel{reedy:eq:7}{{3.16}{16}{weights for latching and matching objects}{equation.3.16}{}}
\newlabel{reedy:lem:sk-rep-reedy}{{3.17}{17}{skeleta of the representables of a Reedy category}{thm.3.17}{}}
\newlabel{reedy:obs:cons-skeleta}{{3.18}{17}{characterising the boundary of a representable}{thm.3.18}{}}
\newlabel{reedy:ex:sequence.latching}{{3.19}{17}{}{thm.3.19}{}}
\newlabel{reedy:ex:pushout.latching}{{3.20}{17}{}{thm.3.20}{}}
\newlabel{reedy:ex:parallel.pair.latching}{{3.21}{18}{}{thm.3.21}{}}
\newlabel{reedy:ex:simp-latching-2}{{3.22}{18}{}{thm.3.22}{}}
\newlabel{reedy:obs:latching.ordinary.colimit}{{3.23}{18}{latching objects as ordinary colimits}{thm.3.23}{}}
\newlabel{reedy:sec:Leibniz-Reedy}{{4}{19}{Leibniz constructions and the Reedy model structure}{section.4}{}}
\newlabel{reedy:obs:box-product}{{4.2}{19}{Leibniz's formula}{thm.4.2}{}}
\newlabel{reedy:defn:leibniz}{{4.4}{20}{the Leibniz construction}{thm.4.4}{}}
\newlabel{reedy:eq:13}{{4.5}{20}{the Leibniz construction}{equation.4.5}{}}
\newlabel{reedy:ex:boundary-prod}{{4.6}{20}{}{thm.4.6}{}}
\newlabel{reedy:obs:leibniz-isos}{{4.7}{20}{Leibniz and structural isomorphisms}{thm.4.7}{}}
\newlabel{reedy:lem:leibniz-cocts}{{4.8}{21}{Leibniz and colimit preservation}{thm.4.8}{}}
\newlabel{reedy:eq:2varadj}{{4.9}{21}{\S \ Leibniz constructions}{equation.4.9}{}}
\newlabel{reedy:lem:leibniz-close}{{4.10}{21}{Leibniz and closures}{thm.4.10}{}}
\newlabel{reedy:obs:leibniz-lifting-properties}{{4.11}{22}{Leibniz and lifting properties}{thm.4.11}{}}
\newlabel{reedy:defn:relative-maps}{{4.14}{22}{relative latching and matching maps}{thm.4.14}{}}
\newlabel{reedy:obs:relative.lifting}{{4.16}{23}{relative latching and matching maps and lifting problems}{thm.4.16}{}}
\newlabel{reedy:eq:i-lift-p}{{4.17}{23}{relative latching and matching maps and lifting problems}{equation.4.17}{}}
\newlabel{reedy:thm:model-structure}{{4.18}{24}{the Reedy model structure}{thm.4.18}{}}
\newlabel{reedy:sec:Leibniz-rel-cell-cx}{{5}{24}{Leibniz constructions and cell complexes}{section.5}{}}
\newlabel{reedy:obs:leibniz-comp}{{5.1}{24}{Leibniz and composites}{thm.5.1}{}}
\newlabel{reedy:defn:transfinite-composites}{{5.3}{25}{transfinite composites}{thm.5.3}{}}
\newlabel{reedy:def:rel-cell}{{5.4}{25}{cell complexes}{thm.5.4}{}}
\newlabel{reedy:eq:10}{{5.5}{26}{cell complexes}{equation.5.5}{}}
\newlabel{reedy:ntn:phi-map}{{5.6}{26}{}{thm.5.6}{}}
\newlabel{reedy:lem:leibniz-tcofp}{{5.7}{26}{Leibniz bifunctors and cell complexes}{thm.5.7}{}}
\newlabel{reedy:eq:11}{{5.8}{27}{Leibniz constructions and cell complexes}{equation.5.8}{}}
\newlabel{reedy:obs:leibniz-tcofp}{{5.9}{27}{}{thm.5.9}{}}
\newlabel{reedy:ex:latch-comp}{{5.10}{28}{relative latching maps of composites II}{thm.5.10}{}}
\newlabel{reedy:cor:leibniz-tcofp}{{5.11}{28}{}{thm.5.11}{}}
\newlabel{reedy:prop:leibniz-tcofp}{{5.12}{28}{}{thm.5.12}{}}
\newlabel{reedy:sec:cellular}{{6}{29}{Cellular presentations and Reedy categories}{section.6}{}}
\newlabel{reedy:obs:two-sided}{{6.1}{29}{skeleta of two-sided representables}{thm.6.1}{}}
\newlabel{reedy:obs:building-skeleta-rep}{{6.2}{29}{building up for skeleta of representables}{thm.6.2}{}}
\newlabel{reedy:prop:building-up}{{6.3}{30}{general building up}{thm.6.3}{}}
\newlabel{reedy:eq:skel-seq}{{6.4}{31}{general building up}{equation.6.4}{}}
\newlabel{reedy:eq:c-cell}{{6.5}{31}{general building up}{equation.6.5}{}}
\newlabel{reedy:eq:skel-seq-cells}{{6.6}{31}{Cellular presentations and Reedy categories}{equation.6.6}{}}
\newlabel{reedy:cor:building-up}{{6.7}{32}{}{thm.6.7}{}}
\newlabel{reedy:cor:B-cell-complex}{{6.8}{32}{}{thm.6.8}{}}
\newlabel{reedy:ex:EZ.simp.set}{{6.9}{33}{}{thm.6.9}{}}
\newlabel{reedy:sec:proof}{{7}{33}{Proof of the Reedy model structure}{section.7}{}}
\newlabel{reedy:lem:triv-cof-char}{{7.1}{33}{}{thm.7.1}{}}
\newlabel{reedy:lem:lifting}{{7.3}{34}{lifting}{thm.7.3}{}}
\newlabel{reedy:lem:factorisation}{{7.4}{34}{factorisation}{thm.7.4}{}}
\newlabel{reedy:eq:factorisation-defn}{{7.5}{35}{Proof of the Reedy model structure}{equation.7.5}{}}
\newlabel{reedy:prop:reedy.cof.gen}{{7.7}{35}{}{thm.7.7}{}}
\newlabel{reedy:sec:hocolim}{{8}{36}{Homotopy limits and colimits}{section.8}{}}
\newlabel{reedy:ex:hocoeq}{{8.2}{37}{homotopy coequalisers}{thm.8.2}{}}
\newlabel{reedy:ex:hoeq}{{8.3}{37}{homotopy equalisers}{thm.8.3}{}}
\newlabel{reedy:prop:reedy.model.dual}{{8.4}{38}{}{thm.8.4}{}}
\newlabel{reedy:ex:mapping}{{8.5}{38}{mapping telescopes}{thm.8.5}{}}
\newlabel{reedy:eq:sequence}{{8.6}{38}{mapping telescopes}{equation.8.6}{}}
\newlabel{reedy:eq:sequence.replacement}{{8.7}{38}{mapping telescopes}{equation.8.7}{}}
\newlabel{reedy:ex:hopushout}{{8.8}{38}{homotopy pushouts}{thm.8.8}{}}
\newlabel{reedy:eq:pushout.compare}{{8.9}{39}{homotopy pushouts}{equation.8.9}{}}
\newlabel{reedy:ex:stupid-simplicial}{{8.10}{39}{}{thm.8.10}{}}
\newlabel{reedy:sec:connected-weights}{{9}{39}{Connected weights}{section.9}{}}
\newlabel{reedy:prop:2/3-SM7}{{9.1}{39}{}{thm.9.1}{}}
\newlabel{reedy:obs:fibrant.constants}{{9.2}{40}{}{thm.9.2}{}}
\newlabel{reedy:cor:connected.weights}{{9.4}{40}{}{thm.9.4}{}}
\newlabel{reedy:sec:simplicial}{{10}{41}{Simplicial model categories and geometric realization}{section.10}{}}
\newlabel{reedy:thm:simp.model.cat}{{10.3}{42}{}{thm.10.3}{}}
\newlabel{reedy:eq:simpmodelreedy}{{10.4}{42}{Simplicial model categories and geometric realization}{equation.10.4}{}}
\newlabel{reedy:obs:geo-filt}{{10.7}{43}{skeletal filtration of geometric realization}{thm.10.7}{}}
\newlabel{reedy:eq:reedy's.po2}{{10.8}{43}{skeletal filtration of geometric realization}{equation.10.8}{}}
\newlabel{reedy:tocindent-1}{0pt}
\newlabel{reedy:tocindent0}{15.01021pt}
\newlabel{reedy:tocindent1}{26.75734pt}
\newlabel{reedy:tocindent2}{0pt}
\newlabel{reedy:tocindent3}{0pt}


==> yoneda_lab.tex <==
\newlabel{yoneda:sec:cosmoi}{{2}{5}{\texorpdfstring {$\infty $}{infinity}-cosmoi}{section.2}{}}
\newlabel{yoneda:ssec:cosmoi}{{2.1}{6}{\texorpdfstring {$\infty $}{infinity}-cosmoi and functors}{subsection.2.1}{}}
\newlabel{yoneda:qcat.ctxt.def}{{2.1.1}{6}{$\infty $-cosmos}{thm.2.1.1}{}}
\newlabel{yoneda:qcat.ctxt:a}{{{{(a)}}}{6}{$\infty $-cosmos}{Item.4}{}}
\newlabel{yoneda:qcat.ctxt:b}{{{{(b)}}}{6}{$\infty $-cosmos}{Item.5}{}}
\newlabel{yoneda:qcat.ctxt:d}{{{{(c)}}}{6}{$\infty $-cosmos}{Item.6}{}}
\newlabel{yoneda:qcat.ctxt:f}{{{{(d)}}}{6}{$\infty $-cosmos}{Item.7}{}}
\newlabel{yoneda:qcat.ctxt:e}{{{{(e)}}}{6}{$\infty $-cosmos}{Item.8}{}}
\newlabel{yoneda:qcat.ctxt.products}{{2.1.2}{6}{}{thm.2.1.2}{}}
\newlabel{yoneda:qcat.ctxt.clarif}{{2.1.3}{6}{}{thm.2.1.3}{}}
\newlabel{yoneda:ex:qcat-qcat-ctxt}{{2.1.4}{7}{the $\infty $-cosmos of quasi-categories}{thm.2.1.4}{}}
\newlabel{yoneda:rec:equiv-and-K}{{2.1.5}{7}{}{thm.2.1.5}{}}
\newlabel{yoneda:rec:equiv-and-K.a}{{{{(a)}}}{7}{}{Item.9}{}}
\newlabel{yoneda:rec:equiv-and-K.b}{{{{(b)}}}{7}{}{Item.10}{}}
\newlabel{yoneda:rec:equiv-and-K.c}{{{{(c)}}}{7}{}{Item.11}{}}
\newlabel{yoneda:rec:equiv-and-K.d}{{{{(d)}}}{7}{}{Item.12}{}}
\newlabel{yoneda:lem:Brown.fact}{{2.1.6}{7}{Brown's factorisation lemma}{thm.2.1.6}{}}
\newlabel{yoneda:obs:Brown.fact.cofibrant}{{2.1.7}{8}{}{thm.2.1.7}{}}
\newlabel{yoneda:lem:isofib-rep}{{2.1.8}{8}{}{thm.2.1.8}{}}
\newlabel{yoneda:defn:qcat-ctxt-functor}{{2.1.9}{9}{}{thm.2.1.9}{}}
\newlabel{yoneda:prop:representable-functors}{{2.1.10}{9}{}{thm.2.1.10}{}}
\newlabel{yoneda:ex:sliced.contexts}{{2.1.11}{9}{sliced $\infty $-cosmoi}{thm.2.1.11}{}}
\newlabel{yoneda:eq:sliced-map}{{2.1.12}{9}{sliced $\infty $-cosmoi}{equation.2.1.12}{}}
\newlabel{yoneda:prop:pullback-functors}{{2.1.13}{10}{pulling back between sliced $\infty $-cosmoi}{thm.2.1.13}{}}
\newlabel{yoneda:ssec:cosmoi-examples}{{2.2}{11}{Examples of \texorpdfstring {$\infty $}{infinity}-cosmoi}{subsection.2.2}{}}
\newlabel{yoneda:lem:model-categories-cosmoi}{{2.2.1}{11}{}{thm.2.2.1}{}}
\newlabel{yoneda:obs:duals-of-cosmoi}{{2.2.2}{11}{}{thm.2.2.2}{}}
\newlabel{yoneda:prop:model-categories-cosmoi}{{2.2.3}{11}{}{thm.2.2.3}{}}
\newlabel{yoneda:ex:cat-cosmos}{{2.2.4}{11}{the $\infty $-cosmos of categories}{thm.2.2.4}{}}
\newlabel{yoneda:ex:CSS-cosmos}{{2.2.5}{12}{the $\infty $-cosmos of complete Segal spaces}{thm.2.2.5}{}}
\newlabel{yoneda:ex:other-CSS-functor}{{2.2.6}{12}{}{thm.2.2.6}{}}
\newlabel{yoneda:ex:segal-cosmos}{{2.2.7}{13}{the $\infty $-cosmos of Segal categories}{thm.2.2.7}{}}
\newlabel{yoneda:ex:marked-cosmos}{{2.2.8}{14}{the $\infty $-cosmos of marked simplicial sets}{thm.2.2.8}{}}
\newlabel{yoneda:prop:rezk-cosmos}{{2.2.9}{14}{the $\infty $-cosmos of Rezk objects}{thm.2.2.9}{}}
\newlabel{yoneda:ex:theta-n-cosmos}{{2.2.10}{16}{the $\infty $-cosmos of $\theta _n$-spaces}{thm.2.2.10}{}}
\newlabel{yoneda:eq:CSS-theta-n-adj}{{2.2.11}{16}{the $\infty $-cosmos of $\theta _n$-spaces}{equation.2.2.11}{}}
\newlabel{yoneda:sec:abstract}{{3}{17}{2-category theory in an \texorpdfstring {$\infty $}{infinity}-cosmos}{section.3}{}}
\newlabel{yoneda:ssec:htpy-2-cat}{{3.1}{17}{The homotopy 2-category of an \texorpdfstring {$\infty $}{infinity}-cosmos}{subsection.3.1}{}}
\newlabel{yoneda:rec:trivial-fibration}{{3.1.3}{18}{equivalences, isofibrations, and surjective equivalences}{thm.3.1.3}{}}
\newlabel{yoneda:lem:isofib.are.representably.so}{{3.1.4}{18}{}{thm.3.1.4}{}}
\newlabel{yoneda:cor:isofib.are.representably.so}{{3.1.5}{19}{}{thm.3.1.5}{}}
\newlabel{yoneda:obs:representing-isos}{{3.1.6}{19}{functors representing invertible 2-cells}{thm.3.1.6}{}}
\newlabel{yoneda:lem:iso-to-weak-equiv}{{3.1.7}{19}{}{thm.3.1.7}{}}
\newlabel{yoneda:prop:equiv.are.weak.equiv}{{3.1.8}{19}{}{thm.3.1.8}{}}
\newlabel{yoneda:obs:bi-coreflection}{{3.1.9}{20}{cofibrant replacement as a {\em bi-coreflection\/}}{thm.3.1.9}{}}
\newlabel{yoneda:ssec:abstract}{{3.2}{20}{Abstract homotopy 2-categories}{subsection.3.2}{}}
\newlabel{yoneda:defn:comma-object}{{3.2.1}{21}{comma object}{thm.3.2.1}{}}
\newlabel{yoneda:eq:comma-square}{{3.2.2}{21}{comma object}{equation.3.2.2}{}}
\newlabel{yoneda:defn:iso-comma-object}{{3.2.3}{22}{iso-comma object}{thm.3.2.3}{}}
\newlabel{yoneda:eq:iso-comma}{{3.2.4}{22}{iso-comma object}{equation.3.2.4}{}}
\newlabel{yoneda:defn:abstract-htpy-2-cat}{{3.2.5}{23}{abstract homotopy 2-category}{thm.3.2.5}{}}
\newlabel{yoneda:ssec:htpy-2-cat-is-abstract}{{3.3}{23}{Comma and iso-comma objects in a homotopy 2-category}{subsection.3.3}{}}
\newlabel{yoneda:lem:htpy-2-cat-commas}{{3.3.1}{23}{}{thm.3.3.1}{}}
\newlabel{yoneda:eq:comma-as-simp-pullback}{{3.3.2}{23}{}{equation.3.3.2}{}}
\newlabel{yoneda:lem:htpy-2-cat-iso-commas}{{3.3.3}{24}{}{thm.3.3.3}{}}
\newlabel{yoneda:eq:iso-comma-as-simp-pullback}{{3.3.4}{24}{}{equation.3.3.4}{}}
\newlabel{yoneda:obs:legs-are-isofibrations}{{3.3.6}{25}{}{thm.3.3.6}{}}
\newlabel{yoneda:ssec:comma}{{3.4}{25}{Stability and uniqueness of comma and iso-comma constructions}{subsection.3.4}{}}
\newlabel{yoneda:defn:span-isofib}{{3.4.1}{25}{}{thm.3.4.1}{}}
\newlabel{yoneda:itm:isofib-right}{{{{(ii)}}}{25}{}{Item.22}{}}
\newlabel{yoneda:itm:isofib-left}{{{{(iii)}}}{25}{}{Item.23}{}}
\newlabel{yoneda:lem:comma-span-isofib}{{3.4.2}{26}{}{thm.3.4.2}{}}
\newlabel{yoneda:eq:span-map}{{3.4.4}{26}{}{equation.3.4.4}{}}
\newlabel{yoneda:lem:equivalence-of-spans}{{3.4.5}{26}{}{thm.3.4.5}{}}
\newlabel{yoneda:obs:ess.unique.1-cell.ind}{{3.4.6}{27}{essential uniqueness of induced 1-cells}{thm.3.4.6}{}}
\newlabel{yoneda:rec:comma-uniqueness}{{3.4.7}{27}{}{thm.3.4.7}{}}
\newlabel{yoneda:lem:comma-uniqueness}{{3.4.8}{28}{stability of (iso-)comma objects under equivalence}{thm.3.4.8}{}}
\newlabel{yoneda:cor:comma-uniqueness}{{3.4.9}{29}{}{thm.3.4.9}{}}
\newlabel{yoneda:lem:comma-composition}{{3.4.10}{29}{}{thm.3.4.10}{}}
\newlabel{yoneda:lem:comma-cancelation}{{3.4.11}{30}{}{thm.3.4.11}{}}
\newlabel{yoneda:lem:restricted-commas-pullback}{{3.4.12}{31}{}{thm.3.4.12}{}}
\newlabel{yoneda:ssec:pullback}{{3.5}{32}{Iso-commas and pullbacks}{subsection.3.5}{}}
\newlabel{yoneda:obs:slice-2-cat}{{3.5.1}{32}{slice 2-categories}{thm.3.5.1}{}}
\newlabel{yoneda:eq:1-cell.in.slice}{{3.5.2}{32}{slice 2-categories}{equation.3.5.2}{}}
\newlabel{yoneda:lem:fibred-equivalence}{{3.5.3}{32}{}{thm.3.5.3}{}}
\newlabel{yoneda:defn:pullback}{{3.5.4}{33}{pullback}{thm.3.5.4}{}}
\newlabel{yoneda:rmk:generalized-1-cell-induction}{{3.5.5}{33}{}{thm.3.5.5}{}}
\newlabel{yoneda:lem:pullbacks-exist}{{3.5.6}{34}{}{thm.3.5.6}{}}
\newlabel{yoneda:defn:pullback-of-an-isofib}{{3.5.7}{34}{}{thm.3.5.7}{}}
\newlabel{yoneda:ex:pullbacks-from-iso-commas}{{3.5.8}{34}{}{thm.3.5.8}{}}
\newlabel{yoneda:ex:old-pullbacks}{{3.5.9}{35}{}{thm.3.5.9}{}}
\newlabel{yoneda:lem:pullback-comp}{{3.5.10}{35}{composition of pullbacks}{thm.3.5.10}{}}
\newlabel{yoneda:ssec:smothering}{{3.6}{36}{Smothering 2-functors and adjunctions}{subsection.3.6}{}}
\newlabel{yoneda:eq:pbk-1-cell}{{3.6.3}{36}{}{equation.3.6.3}{}}
\newlabel{yoneda:eq:pbk-2-cell}{{3.6.4}{37}{}{equation.3.6.4}{}}
\newlabel{yoneda:lem:pullback-smothering}{{3.6.5}{37}{}{thm.3.6.5}{}}
\newlabel{yoneda:cor:adjunctions-pullback}{{3.6.6}{37}{}{thm.3.6.6}{}}
\newlabel{yoneda:cor:pullback-uniqueness}{{3.6.7}{37}{}{thm.3.6.7}{}}
\newlabel{yoneda:defn:iso-comma-slice-2-cat}{{3.6.8}{38}{}{thm.3.6.8}{}}
\newlabel{yoneda:eq:iso-comma-1-cell}{{3.6.9}{38}{}{equation.3.6.9}{}}
\newlabel{yoneda:eq:iso-comma-2-cell}{{3.6.10}{38}{}{equation.3.6.10}{}}
\newlabel{yoneda:lem:iso-comma-smothering}{{3.6.11}{38}{}{thm.3.6.11}{}}
\newlabel{yoneda:cor:adjunctions-iso-comma}{{3.6.12}{39}{}{thm.3.6.12}{}}
\newlabel{yoneda:obs:adj.rep.def}{{3.6.13}{39}{adjunctions are representably defined}{thm.3.6.13}{}}
\newlabel{yoneda:obs:RARI}{{3.6.14}{39}{right adjoint right inverse}{thm.3.6.14}{}}
\newlabel{yoneda:obs:gen.2-cat.results}{{3.6.15}{40}{}{thm.3.6.15}{}}
\newlabel{yoneda:sec:cartesian}{{4}{40}{Cartesian fibrations}{section.4}{}}
\newlabel{yoneda:ssec:cartesian}{{4.1}{40}{Cartesian fibrations}{subsection.4.1}{}}
\newlabel{yoneda:defn:weak.cart.2-cell}{{4.1.1}{40}{cartesian 2-cells}{thm.4.1.1}{}}
\newlabel{yoneda:itm:weak.cart.i}{{{{(i)}}}{40}{cartesian 2-cells}{Item.38}{}}
\newlabel{yoneda:itm:weak.cart.ii}{{{{(ii)}}}{40}{cartesian 2-cells}{Item.39}{}}
\newlabel{yoneda:obs:cart.iso.stab}{{4.1.2}{41}{isomorphism stability}{thm.4.1.2}{}}
\newlabel{yoneda:obs:weak.cart.conserv}{{4.1.3}{41}{more conservativity}{thm.4.1.3}{}}
\newlabel{yoneda:defn:cart-fib}{{4.1.4}{41}{cartesian fibration}{thm.4.1.4}{}}
\newlabel{yoneda:eq:2-cell.to.lift}{{4.1.5}{41}{cartesian fibration}{equation.4.1.5}{}}
\newlabel{yoneda:obs:weak.cart.lift.unique}{{4.1.6}{41}{uniqueness of cartesian lifts}{thm.4.1.6}{}}
\newlabel{yoneda:prop:cart-fib-comp}{{4.1.7}{42}{composites of cartesian fibrations}{thm.4.1.7}{}}
\newlabel{yoneda:ntn:for.commas}{{4.1.8}{42}{}{thm.4.1.8}{}}
\newlabel{yoneda:lem:adj.for.commas}{{4.1.9}{43}{}{thm.4.1.9}{}}
\newlabel{yoneda:thm:cart.fib.chars}{{4.1.10}{44}{}{thm.4.1.10}{}}
\newlabel{yoneda:itm:cart.fib.chars.i}{{{{(i)}}}{44}{}{Item.42}{}}
\newlabel{yoneda:itm:cart.fib.chars.ii}{{{{(ii)}}}{44}{}{Item.43}{}}
\newlabel{yoneda:eq:cartesian.fib.adj}{{4.1.11}{44}{}{equation.4.1.11}{}}
\newlabel{yoneda:itm:cart.fib.chars.iii}{{{{(iii)}}}{44}{}{Item.44}{}}
\newlabel{yoneda:eq:cartesian.isosect.adj}{{4.1.12}{44}{}{equation.4.1.12}{}}
\newlabel{yoneda:obs:fibered-unit-iso}{{4.1.13}{44}{}{thm.4.1.13}{}}
\newlabel{yoneda:obs:constructing-weak-lifts}{{4.1.14}{45}{}{thm.4.1.14}{}}
\newlabel{yoneda:cor:cart-fib-rep}{{4.1.15}{45}{}{thm.4.1.15}{}}
\newlabel{yoneda:ex:domain-fibration}{{4.1.16}{45}{}{thm.4.1.16}{}}
\newlabel{yoneda:obs:domain-cart-lifts}{{4.1.17}{46}{cartesian lifts for domain projections}{thm.4.1.17}{}}
\newlabel{yoneda:ex:general-domain-projection}{{4.1.18}{47}{}{thm.4.1.18}{}}
\newlabel{yoneda:prop:bifibration-adjunction}{{4.1.20}{47}{}{thm.4.1.20}{}}
\newlabel{yoneda:eq:pseudo-slice-adj}{{4.1.21}{48}{Cartesian fibrations}{equation.4.1.21}{}}
\newlabel{yoneda:eq:RARI-lifting}{{4.1.24}{49}{right adjoint right inverse as a lifting property}{equation.4.1.24}{}}
\newlabel{yoneda:cor:lurie-cartesian}{{4.1.24}{50}{}{thm.4.1.24}{}}
\newlabel{yoneda:eq:lurie-cartesian}{{4.1.25}{50}{}{equation.4.1.25}{}}
\newlabel{yoneda:ssec:groupoidal}{{4.2}{51}{Groupoidal cartesian fibrations}{subsection.4.2}{}}
\newlabel{yoneda:defn:groupoidal-object}{{4.2.1}{51}{groupoidal objects}{thm.4.2.1}{}}
\newlabel{yoneda:lem:groupoidal.conserv}{{4.2.2}{51}{}{thm.4.2.2}{}}
\newlabel{yoneda:cor:groupoidal-cart-fib-rep}{{4.2.4}{51}{}{thm.4.2.4}{}}
\newlabel{yoneda:prop:groupoidal-ext-char}{{4.2.5}{51}{}{thm.4.2.5}{}}
\newlabel{yoneda:lem:gpd-cart-cancel}{{4.2.6}{52}{}{thm.4.2.6}{}}
\newlabel{yoneda:prop:iso-groupoidal-char}{{4.2.7}{52}{}{thm.4.2.7}{}}
\newlabel{yoneda:obs:biterminal}{{4.2.10}{53}{biterminal objects in the homotopy 2-category}{thm.4.2.10}{}}
\newlabel{yoneda:ex:groupoidal-representable}{{4.2.11}{54}{}{thm.4.2.11}{}}
\newlabel{yoneda:sec:stability}{{5}{54}{Cartesian functors and pullbacks of cartesian fibrations}{section.5}{}}
\newlabel{yoneda:itm:to-do-cart-cells}{{{{(i)}}}{54}{Cartesian functors and pullbacks of cartesian fibrations}{Item.45}{}}
\newlabel{yoneda:itm:to-do-pullback}{{{{(ii)}}}{54}{Cartesian functors and pullbacks of cartesian fibrations}{Item.46}{}}
\newlabel{yoneda:ssec:cart-fun}{{5.1}{54}{Cartesian functors}{subsection.5.1}{}}
\newlabel{yoneda:eq:cartesian-functor-square}{{5.1.2}{54}{}{equation.5.1.2}{}}
\newlabel{yoneda:thm:cart.fun.chars}{{5.1.4}{55}{}{thm.5.1.4}{}}
\newlabel{yoneda:itm:cart.fun.chars.i}{{{{(i)}}}{55}{}{Item.47}{}}
\newlabel{yoneda:itm:cart.fun.chars.ii}{{{{(ii)}}}{55}{}{Item.48}{}}
\newlabel{yoneda:eq:cart-fun-iso.ii}{{5.1.5}{55}{}{equation.5.1.5}{}}
\newlabel{yoneda:itm:cart.fun.chars.iii}{{{{(iii)}}}{55}{}{Item.49}{}}
\newlabel{yoneda:eq:cart-fun-iso.iii}{{5.1.6}{55}{}{equation.5.1.6}{}}
\newlabel{yoneda:cor:radj-cartesian}{{5.1.7}{57}{}{thm.5.1.7}{}}
\newlabel{yoneda:lem:cart-arrows-compose}{{5.1.8}{58}{}{thm.5.1.8}{}}
\newlabel{yoneda:lem:cart-arrows-cancel}{{5.1.9}{58}{}{thm.5.1.9}{}}
\newlabel{yoneda:ssec:pullback-stability}{{5.2}{59}{Pullback stability}{subsection.5.2}{}}
\newlabel{yoneda:prop:cart-fib-pullback}{{5.2.1}{59}{pullbacks of cartesian fibrations}{thm.5.2.1}{}}
\newlabel{yoneda:cor:groupoidal-pullback}{{5.2.2}{61}{}{thm.5.2.2}{}}
\newlabel{yoneda:sec:yoneda}{{6}{62}{The Yoneda lemma}{section.6}{}}
\newlabel{yoneda:thm:yoneda}{{6.0.1}{62}{Yoneda lemma}{thm.6.0.1}{}}
\newlabel{yoneda:eq:evaluation-comma-adjunction}{{6.0.2}{62}{The Yoneda lemma}{equation.6.0.2}{}}
\newlabel{yoneda:ssec:pullback-functoriality}{{6.1}{62}{Functoriality of pullbacks of cartesian fibrations}{subsection.6.1}{}}
\newlabel{yoneda:defn:pbshape-2-cat}{{6.1.1}{63}{}{thm.6.1.1}{}}
\newlabel{yoneda:eq:1-cell-in-pbshape}{{6.1.2}{63}{}{equation.6.1.2}{}}
\newlabel{yoneda:eq:cartesian-weak-pullback}{{6.1.3}{63}{Functoriality of pullbacks of cartesian fibrations}{equation.6.1.3}{}}
\newlabel{yoneda:defn:square-2-cat}{{6.1.4}{63}{}{thm.6.1.4}{}}
\newlabel{yoneda:eq:1-cell-in-square}{{6.1.5}{63}{}{equation.6.1.5}{}}
\newlabel{yoneda:prop:cartesian-smothering}{{6.1.6}{64}{}{thm.6.1.6}{}}
\newlabel{yoneda:ssec:proof-yoneda}{{6.2}{64}{Proof of the Yoneda lemma}{subsection.6.2}{}}
\newlabel{yoneda:eq:1-cell-in-lax-comma}{{6.2.2}{64}{lax slice 2-category}{equation.6.2.2}{}}
\newlabel{yoneda:obs:lax-slice-adjunction}{{6.2.3}{65}{}{thm.6.2.3}{}}
\newlabel{yoneda:eq:lax-slice-left-adjoint}{{6.2.4}{65}{}{equation.6.2.4}{}}
\newlabel{yoneda:obs:pullback-2-category}{{6.2.5}{65}{}{thm.6.2.5}{}}
\newlabel{yoneda:lem:rep-cart-cells}{{6.2.6}{65}{}{thm.6.2.6}{}}
\newlabel{yoneda:eq:strange-right-adjoint}{{6.2.7}{66}{Proof of the Yoneda lemma}{equation.6.2.7}{}}
\newlabel{yoneda:eq:unrestricted-adjunction}{{6.2.8}{66}{Proof of the Yoneda lemma}{equation.6.2.8}{}}
\newlabel{yoneda:lem:codomain-restriction}{{6.2.9}{66}{}{thm.6.2.9}{}}
\newlabel{yoneda:eq:chi-lifting-phi}{{6.2.10}{67}{Proof of the Yoneda lemma}{equation.6.2.10}{}}
\newlabel{yoneda:eq:restricted-adjunction}{{6.2.11}{67}{Proof of the Yoneda lemma}{equation.6.2.11}{}}
\newlabel{yoneda:lem:last-yoneda-step}{{6.2.12}{67}{}{thm.6.2.12}{}}
\newlabel{yoneda:cor:groupoidal-yoneda}{{6.2.13}{68}{}{thm.6.2.13}{}}
\newlabel{yoneda:sec:appendix}{{7}{68}{Appendix: proof of Theorem~\ref {thm:cart.fib.chars}}{section.7}{}}
\newlabel{yoneda:itm:cart.fib.chars.i'}{{{{(i)}}}{68}{}{Item.50}{}}
\newlabel{yoneda:itm:cart.fib.chars.ii'}{{{{(ii)}}}{68}{}{Item.51}{}}
\newlabel{yoneda:eq:cartesian.fib.adj'}{{7.0.1}{69}{}{equation.7.0.1}{}}
\newlabel{yoneda:itm:cart.fib.chars.iii'}{{{{(iii)}}}{69}{}{Item.52}{}}
\newlabel{yoneda:eq:cartesian.isosect.adj'}{{7.0.2}{69}{}{equation.7.0.2}{}}
\newlabel{yoneda:ntn:adj.for.commas}{{7.0.3}{69}{}{thm.7.0.3}{}}
\newlabel{yoneda:eq:compat.sq.1}{{7.0.4}{71}{Appendix: proof of Theorem~\ref {thm:cart.fib.chars}}{equation.7.0.4}{}}
\newlabel{yoneda:eq:defn.muhat}{{7.0.5}{71}{Appendix: proof of Theorem~\ref {thm:cart.fib.chars}}{equation.7.0.5}{}}
\newlabel{yoneda:tocindent-1}{0pt}
\newlabel{yoneda:tocindent0}{15.01021pt}
\newlabel{yoneda:tocindent1}{20.88377pt}
\newlabel{yoneda:tocindent2}{34.49158pt}
\newlabel{yoneda:tocindent3}{0pt}

